Minmax Regret for sink location on paths with general capacities

In dynamic flow networks, every vertex starts with items (flow) that need to be shipped to designated sinks. All edges have two associated quantities: length, the amount of time required for a particle to traverse the edge, and capacity, the number of units of flow that can enter the edge in unit time. The goal is move all flow to the sinks. A variation of the problem, modelling evacuation protocols, is to find the sink location(s) that minimize evacuation time, restricting the flow to be CONFLUENT. Solving this problem is is NP-hard on general graphs, and thus research into optimal algorithms has traditionally been restricted to special graphs such as paths, and trees. A specialized version of robust optimization is minmax REGRET, in which the input flows at the vertices are only partially defined by constraints. The goal is to find a sink location that has the minimum{ regret} over all input flows that satisfy the partially defined constraints. Regret for a fully defined input flow and a sink is defined to be the difference between the evacuation time to that sink and the optimal evacuation time. A large recent literature derives polynomial time algorithms for the minmax regret $k$-sink location problem on paths and trees under the simplifying condition that all edges have the same (uniform) capacity. This paper develops a $O(n^4 \log n)$ time algorithm for the minmax regret $1$-sink problem on paths with general (non-uniform) capacities. To the best of our knowledge, this is the first minmax regret result for dynamic flow problems in any type of graph with general capacities.

==> algorithm.tex <==
\section{Algorithm}
\label{sec:algorithm}

The approach followed is to evaluate  $R_{\max}(P,x)$   
using  \Cref  {thm:reduction3}   by noting that the values introduced in 
\Cref{def:gandh defs}  are actually the maximum values over piecewise linear functions and then derive efficient ways of calculating those maximal values.

$R_{OPT}(P)$ will then be found  find via a binary search on unimodal $R_{\max}(P,x)$. 



\subsection{Upper Envelopes}
Our algorithms  will use the following simple Lemmas and Observations.



\begin{definition}
Let 
$f_i(x) = m_i x + b_i$, $1 \le i \le t$  be  a set of lines.
Their {\em upper envelope} is the function
$$f(x) = \max_{1 \le i \le t} f_i(x).$$
The set of lines is {\em sorted} if  $0 \le m_ 1 \le m_2 \le \cdots \le m_t$.  
\end{definition}

\begin{observation}
\label{obs:ue}
Let $I=[\ell,r]$ be some interval,  $f_i(x)$ a sorted set of $m$ lines and $f(x)$ their upper envelope.
Then there exists a sequence of $t' \le t$ indices,
$ 1 \le i_1 < i_2 < \cdots < i_{t'}  \le  t$ and a sequence of  $t'+1$  points $\ell= q_0 < q_1  < q_2 \cdots <q_{t'} = r$ such that
$$\forall x \in  [q_{j-1}, q_j],\quad 
f(x) = f_{i_j}(x).
$$
The $q_j$ are the {\em critical points} or {\em inflection points}  of the upper envelope and they and the $i_j$ can be found in $O(m)$ time.
\end{observation}



\begin{lemma}
\label{lem:env} Let $s$ be any fixed scenario. Recall the definition of  $s_{-i}(z)$    from \Cref{def:sstuff}.
Let $x$ be  any fixed sink location. 

Then 
$\Theta_L(P,x: s_{-i} (z))$,  $\Theta_R(P,x: s_{-i} (z))$ and $\Theta (P,x: s_{-i} (z))$ are all, as a function of $z$, upper envelopes of a set of lines, all with nonnegative slope.  
these functions all have $O(n)$ critical points and  these critical  points and the 
 line equations of the upper envelopes can be calculated in $O(n)$ time.
\end{lemma}
\begin{proof}
%Recall the definitions of the evacuation times in \Cref{eq:Theta Def,eq:evac,eq:evaca}.
%We first examine  $\Theta_L(P,x: s_{-i} (z))$. 
%
%
%If $x \le x_i$ then $\Theta_L(P,x: s_{-i} (z))=\Theta_L(P,x: s)$  is a constant and can be calculated in $O(n)$ time.

%Assume then that $x_i < x$   %Without loss of generality also assume that $x_i < x$ (the other case is symmetric). 
Let $t = \max\{j \,: x_j < x\}.$
From the definitions of the evacuation times in \Cref{eq:Theta Def,eq:evac,eq:evaca} and
%Next note that  $\beta = \Theta_R(P,x: s_{-i} (z))$ is a constant that can be calculated in $O(n)$ time.  
%Plugging into 
\Cref{lem:evac},
\begin{equation}
\label{eq:gUE}
\Theta_L(P,x: s_{-i} (z)) =\max_{0 \le j  \le  t} g_j(x :s_{-i}(z))
\end{equation}
where, after setting  $\alpha_j = \frac 1  {\tilde c_{j,t}}$, 
$$g_j(x :s_{-i}(z)) = d(x_j,x) %+ \frac{W_{0,j}(s_{-i} (z))} {\min\{ c_v \,:\, j \le v \le t\}}
+ \frac{W_{0,j}(s_{-i} (z))}  {\tilde c_{j,t}}
= d(x_j,x) +  \alpha_j W_{0,j}(s_{-i} (z)).
$$
Note that the  $\alpha_j$ are  nonnegative nonincreasing in $j$ and can be calculated in order in a total $O(n)$ time using a linear scan.
Finally note 
$$
W_{0,j}(s_{-i} (z)) = \sum_{v=0}^j w_v\left(s_{-i}(z)\right) =
\left\{
\begin{array}{ll}
 \sum_{v=0}^j w_v(s) = W_{0,j}(s) & \mbox{if $j < i$},\\
 z  - w_i(s) +  \sum_{v=0}^j w_v(s) = z - w_i(s) + W_{0,j}(s), & \mbox{if $j  \ge i$}.
\end{array}
\right.
$$
Thus
$$
g_j(s_{-i}(z))=
\left\{
\begin{array}{ll}
 \alpha_j  W_{0,j}(s) + d(x_i,x) & \mbox{if $j < i$},\\
 \alpha_j z  + (d(x_i,x) - \alpha_j w_i(s) +\alpha_j  W_{0,j}(s))    & \mbox{if $j  \ge i$}.\
\end{array}
\right.
$$
The $g_j(s_{-i}(z))$ with $ j < i$ are constants (lines with slope zero).
% and can each be calculated in $O(1)$ time. 
The $g_j(s_{-i}(z))$ with $ j \ge  i$ are lines in $z$ with slopes given in non-increasing order.  From
\Cref{eq:gUE}, $\Theta_L(P,x: s_{-i} (z))$ is the  upper envelope of those lines..  Reversing the order of these lines puts them in exactly the format of 
\Cref{obs:ue} and thus $\Theta_L(P,x: s_{-i} (z))$ and its critical points and defining line segments can be found in $O(n)$ time.

\medskip

 The analysis of $\Theta_R(P,x: s_{-i} (z))$ is symmetric and exactly the same.

\medskip
Since 
$$\Theta(P,x: s_{-i} (z)) = \max\bigl( \Theta_L(P,x: s_{-i} (z)),\,  \Theta_R(P,x: s_{-i} (z)) \bigr),$$
it is the maximum  of the two upper envelopes of lines and is therefore  the upper envelope of the original  $O(n)$ lines.
Also, it   can be built from the left and right  upper envelopes by a simple merge in $O(n)$ time.
\end{proof}

\begin{definition}
\label{def:UE LE}
Let $i$  be an index  and $s$ a scenario with $w_i(s)=0.$ 
Let $t ,j$ be indices and set 
 $d_{t,j} = |x_j - x_t|$
  and  $W_{t,j} = \sum_{k=t}^j w_t(s).$
For  $\alpha \ge 0$ and $ t\le j$ set 
$$W_{t,j}(\alpha)
= \sum_{k=t}^j w_k\left(s_{-i}(\alpha) \right)=
\left\{
\begin{array}{ll}
W_{t,j} & \mbox{if  $i< t$ or $j < i$}\\
W_{t,j} + \alpha & \mbox{if $t \le i \le j$ }
\end{array}
\right.
$$
Define
\begin{align*}
\lue_{i,j}(\alpha) &=  \Theta_L(P,x_j :s_{-i} (\alpha)) &= \max_{0 \le t <j}  g_t(x_j:s_{-i} (\alpha))   &= \max_{0 \le t <j}  \left( d_{t,j}  +  \frac 1 {\tc_{t,j}}W_{0,t}(\alpha) \right) \\
\rue_{i,j}(\alpha) &=  \Theta_R(P,x_j :s_{-i} (\alpha))&=  \max_{j < t \le n}  h_t(x_j:s_{-i} (\alpha))      &=  \max_{j < t \le n}  \left(  d_{j,t}+  \frac 1 {\tc_{j,t}}W_{t,n}(\alpha)\right)
\end{align*}
We say that 
\begin{itemize}
\item {\em Line $t$ is on $\lue_{i,j}$} if  $\exists \alpha_1 < \alpha_2$ such that, $\forall \alpha \in [\alpha_1,\alpha_2],$
$\lue_{i,j}(\alpha)  = g_t(x_j:s_{-i} (\alpha)) $
\item  {\em Line $t$ is on $\rue_{i,j}$} if $\exists \alpha_1 < \alpha_2$ such that, $\forall \alpha \in [\alpha_1,\alpha_2],$
$\rue_{i,j}(\alpha)  = h_t(x_j:s_{-i} (\alpha)).$ 
\end{itemize}
\end{definition}



\begin{observation}
\label{obs:LUE}
The definitions and \Cref {lem:env}   immediately imply
\begin{itemize}
\item 
As functions of $\alpha,$   $\lue_{i,j}(\alpha)$  and $\rue_{i,j}(\alpha)$  are  upper envelopes, respectively, of $j$ and 
  $n-j$ lines. 

 \item Let $t$ be the index such that, $\lue_{i,j}(\alpha)=g_t(x_j:s_{-i} (\alpha))$   and $t'$ the index such that 
$\rue_{i,j}(\alpha)= h_{t'}(x_j:s_{-i} (\alpha))$.  Then 
 $t=\lcrv(x_j: s_{-i} (\alpha))$ and $t' = \rcrv(x_j: s_{-i} (\alpha))$.
\end{itemize}
 \end{observation}
 \begin{lemma}
 \label{lem:crv change}
 Fix index $i$.  Then
 \begin{enumerate}
 \item \ 
 $$\forall y,\ \forall \alpha' > \alpha \ge 0,\quad
 \lcrv(y: s_{-i} (\alpha')) \le \lcrv(y: s_{-i} (\alpha)).$$
 \item  If $y' < y$  then $$\forall \alpha \ge 0,\quad \lcrv(y': s_{-i} (\alpha)) \le \lcrv(y: s_{-i} (\alpha)).$$
 \end{enumerate}
 \end{lemma}
 
 \begin{proof}
 
 To prove (1) note that  $\lue_{i,j}(z)$ is an upper envelope of lines. Slopes do not decrease on an upper envelope of lines so the  slope at  $\lue_{i,j}(\alpha)$ is less than equal to the slope at 
 $\lue_{i,j}(\alpha')$.  
 
 Working through the definitions, the slope of the line at value $z$ will be  $\frac 1 {\tc_{j,t}}$ where
 $t = \lcrv(y: s_{-i} (z)).$ Now note that $\tc_{j,t}$ is non-decreasing in $t$ so 
 $\frac 1 {\tc_{j,t}}$  is non-increasing in $t$, proving (1).
 
 
 
 
 
 
% To prove (1), fix $y$.
%
%Now let $t_1 \le t_2$ such that $x_{t_2} \le y$ and assume that
%$$ g_{t_1}(y:s_{-i} (\alpha))   \ge g_{t_2}(y:s_{-i} (\alpha)).$$
%Then 
%
%\begin{eqnarray*}
%\label{eq:gtstart}
%   d(x_{t_1},y) +  \frac 1 {\tc_{t_1,y}}  W_{0,t_1}(\alpha)    &=& g_{t_1}(y:s_{-i} (\alpha))\\
%   									&\ge& g_{t_2}(y:s_{-i} (\alpha))\\
%   									&=&     d(x_{t_2},y) +  \frac 1 {\tc_{t_2,j}} W_{0,t_2}(\alpha).
%\end{eqnarray*}
%Next note that
%$$W_{0,t_1}(\alpha')  - W_{0,t_1}(\alpha) 
%=
%\left\{
%\begin{array}{ll}
%\alpha & \mbox { if $t_1 \le i$.}\\
%0  & \mbox { if $t_1 > i$.}
%\end{array}
%\right.,\quad
%W_{0,t_2}(\alpha')  - W_{0,t_2}(\alpha) 
%=
%\left\{
%\begin{array}{ll}
%\alpha & \mbox { if $t_2 \le i$.}\\
%0  & \mbox { if $t_2 > i$.}
%\end{array}
%\right..
%$$
%Since $t_1 \le t_2$ this shows that
%$$W_{0,t_1}(\alpha')  - W_{0,t_1}(\alpha)  \ge W_{0,t_1=2}(\alpha')  - W_{0,t_2}(\alpha).$$
%By definition, ${\tc_{t_1,y}} \le {\tc_{t_2,y}}$. Thus , we have just shown that
%\begin{equation}
%\label{eq:gtstart3}
%\forall \alpha' > \alpha,\,\quad
%g_{t_1}(y:s_{-i} (\alpha))  \ge  g_{t_2}(y:s_{-i} (\alpha))
%  \quad\Rightarrow\quad  g_{t_1}(y:s_{-i} (\alpha'))   \ge g_{t_2}(y:s_{-i} (\alpha')).
%\end{equation}
%
%Now set $t_1 =\lcrv(y: s_{-i} (\alpha))$ and  $t_2= \lcrv(y: s_{-i} (\alpha'))$.
%
%If $\lcrv(y: s_{-i} (\alpha')) >  \lcrv(y: s_{-i} (\alpha))$ then $t_1 < t_2 < y.$
%
%By the definition of $t_1$ and $t_2$ we have
%$$g_{t_1}(y:s_{-i} (\alpha))  \ge  g_{t_2}(y:s_{-i} (\alpha))$$
%but
%$$g_{t_1}(y:s_{-i} (\alpha'))   < g_{t_2}(y:s_{-i} (\alpha')).$$
%This contradicts \Cref{eq:gtstart3} and thus  is impossible so we must have
%$ \lcrv(y: s_{-i} (\alpha')) \le   \lcrv(y: s_{-i} (\alpha))$, completing the proof of (1).
%
%

\medskip

The complication in proving  (2) is that  as $y$ moves to the right  the upper envelope composing  $\Theta_L(P, y :s_{-i} (\alpha))$ can change dramatically.  Not only do new items need to be evacuated to $y$, but the slopes of old lines might be changed.

To prove (2)  we split into three steps.

\medskip

 \par\noindent\underline{Step 1:}  If $\exists j$ such that  that $x_j < y' < y \le x_{j+1}$
 then $ \lcrv(y': s_{-i} (\alpha)) = \lcrv(y: s_{-i} (\alpha)).$\\
 To see this note from \Cref{cor:smooth evac}  that, for  $s=s_{-i} (\alpha),$
$$\Theta_L(P,y:s) = \Theta_L(P,x_{j+1}:s)  - (x_{j+1}- y),\quad
\Theta_L(P,y:s) = \Theta_L(P,x_{j+1}:s)  - (x_{j+1}- y'),
$$
so 
$$ \lcrv(y': s_{-i} (\alpha)) = \lcrv(y: s_{-i} (\alpha)).$$

\medskip

 \par\noindent\underline{Step 2:} We will actually prove that 
 \begin{equation}
 \label{eq:lcvrdown}
  \lcrv(x_j: s_{-i} (\alpha)) \le  \lcrv(x_{j+1}: s_{-i} (\alpha)).
  \end{equation}


%
%Now let $t_1 \le t_2$ such that $x_{t_2} \le y$ and assume that
%$$ g_{t_1}(y:s_{-i} (\alpha))   \ge g_{t_2}(y:s_{-i} (\alpha)).$$
%Then 
%
%\begin{eqnarray*}
%\label{eq:gtstart}
%   d(x_{t_1},y) +  \frac 1 {\tc_{t_1,y}}  W_{0,t_1}(\alpha)    &=& g_{t_1}(y:s_{-i} (\alpha))\\
%  									&\ge& g_{t_2}(y:s_{-i} (\alpha))\\
%   									&=&     d(x_{t_2},y) +  \frac 1 {\tc_{t_2,j}} W_{0,t_2}(\alpha).
%\end{eqnarray*}


%Then
% Then, for all $t < y'$, ${\tc_{t,y}} = {\tc_{t,j}} = {\tc_{t,y'}}.$  Thus
%\begin{eqnarray*}
%g_t(y':s_{-i} (\alpha))  &=&   d(x_t,y') +  \frac 1 {\tc_{t,j}} W_{0,t}(\alpha)\\
%                                 & =&  (y'-y) + d(x_t,y) +  \frac 1 {\tc_{t,j}} W_{0,t}(\alpha)\\
%                                 &=&  (y'-y)+ g_t(y:s_{-i} (\alpha)).
%                                 \end{eqnarray*}
%Thus, we have just shown that,  $\forall \alpha \ge 0,$  for all $t_1 < t_2 \le x_j,$
%\begin{equation}
%\label{eq:gstart4}
%g_{t_1}(y:s_{-i} (\alpha))   \ge g_{t_2}(y:s_{-i} (\alpha))
%\quad
%\mbox{if and only if}
%\quad 
%g_{t_1}(y':s_{-i} (\alpha))   \ge g_{t_2}(y':s_{-i} (\alpha)).
%\end{equation}

 To do this we will  prove that if  $t_1  <  t_2 \le x_j$ then
 $$
 g_{t_1}(x_j:s_{-i} (\alpha))   \le  g_{t_2}(x_j:s_{-i} (\alpha))
 \quad \Rightarrow\quad
 g_{t_1}(x_{j+1}:s_{-i} (\alpha))   \le g_{t_2}(x_{j+1}:s_{-i} (\alpha)).$$
 To see that this implies \Cref{eq:lcvrdown}
 %note first that
 %if $\lcrv(x_{j+1}: s_{-i} (\alpha))= j+1$ then \Cref{eq:lcvrdown} is trivially true.
let $t_2 = \lcrv(x_j: s_{-i} (\alpha)) \le j.$  

Then, by definition, $\forall t_1 < t_2$,
 $g_{t_1}(x_j:s_{-i} (\alpha))   \le  g_{t_2}(x_j:s_{-i} (\alpha))$.
 
 Our statement then   implies 
 $\forall t_1 < t_2$,
 $g_{t_1}(x_{j+1}:s_{-i} (\alpha))   \le  g_{t_2}(x_{j+1}:s_{-i} (\alpha))$,
further  implying  $ t_2 \le \lcrv(x_{j+1}: s_{-i} (\alpha)) \le j$.

 
 
 For this case note that,  
 \begin{eqnarray*}
g_{t_1}(x_j :s_{-i} (\alpha))  &=&  d(x_{t_1},x_j) +  \frac 1 {\tc_{t_1,j}} W_{0,t_1}(\alpha) \\
g_{t_2}(x_j:s_{-i} (\alpha))  &=&   d(x_{t_2},x_j) +  \frac 1 {\tc_{t_2,j}} W_{0,t_2}(\alpha),
\end{eqnarray*}
and
\begin{eqnarray*}
g_{t_1}(x_{j+1} :s_{-i} (\alpha))  &=&  d_j + d(x_{t_1},x_j) +  \frac 1 {\tc_{t_1,j+1}} W_{0,t_1}(\alpha) \\
g_{t_2}(x_{j+1} :s_{-i} (\alpha))  &=&  d_j + d(x_{t_2},x_j) +  \frac 1 {\tc_{t_2,j+1}} W_{0,t_2}(\alpha).
\end{eqnarray*}




There are now three possibilities. In each of them we will assume $t_1 < t_2$ and 
 $g_{t_1}(x_j:s_{-i} (\alpha))   \le  g_{t_2}(x_j:s_{-i} (\alpha))$
and then show that that implies 
 $g_{t_1}(x_{j+1}:s_{-i} (\alpha))   \le g_{t_2}(x_{j+1}:s_{-i} (\alpha)).$
\medskip

\par\noindent{\bf (a) $\bf {\tc_{t_1,j}}= {\tc_{t_1,j+1}}$ and  $\bf {\tc_{t_2,j}}= {\tc_{2_1,j+1}}$:}

\smallskip

In this case, trivially,
\begin{eqnarray*}
g_{t_1}(x_{j+1}:s_{-i} (\alpha))   
&=& d_j +g_{t_1}(x_{j}:s_{-i} (\alpha))\\
&\le& d_j +g_{t_2}(x_{j}:s_{-i} (\alpha))\\
&=& g_{t_2}(x_{j+1}:s_{-i} (\alpha))\\   
&\le& g_{t_2}(x_{j-1}:s_{-i} (\alpha)).
\end{eqnarray*}

\par\noindent{\bf (b) $\bf {\tc_{t_1,j}} = {\tc_{t_1,j+1}}$  and  $\bf {\tc_{t_2,j}}  \not= {\tc_{t_2,j+1}}$:}

\smallskip
Note that this means that  ${\tc_{t_2,j}}  >  {\tc_{t_2,j+1}}= c_j$. Thus
\begin{eqnarray*}
g_{t_1}(x_{j+1} :s_{-i} (\alpha)) 
						&=&  d_j + g_{t_1}(x_j :s_{-i} (\alpha))\\
						&\le&  d_j+ g_{t_2}(x_j :s_{-i} (\alpha))\\
  						&=&  d_j+ d(x_{t_2},x_j) +  \frac 1 {\tc_{t_2,j}} W_{0,t_2}(\alpha) \\
						&\le&  d_j+ d(x_{t_2},x_j) +  \frac 1 {\tc_{t_2,j+1}} W_{0,t_2}(\alpha) \\
						&=&  g_{t_2}(x_{j+1} :s_{-i} (\alpha)).
\end{eqnarray*}
\medskip


\par\noindent{\bf  (c) $\bf {\tc_{t_1,j}} \not= {\tc_{t_1,j+1}}$  and  $\bf {\tc_{t_2,j}}  \not= {\tc_{2_1,j+1}}$:}


\smallskip

This can only happen if  ${\tc_{t_2,j+1}} = {\tc_{t_1,j+1}} < {\tc_{t_1,j}}  < {\tc_{t_2,j}}$, which,. together with the fact that $W_{0,t_1}(\alpha) \le W_{0,t_2}(\alpha)$
immediately implies
$$ \left(\frac 1 {\tc_{t_1,j+1}} -   \frac 1 {\tc_{t_1,j}} \right)  W_{0,t_1}(\alpha)\left(   \le   \frac 1 {\tc_{t_1,j+1}} -   \frac 1 {\tc_{t_2,j}}\right)W_{0,t_2}(\alpha).$$
%This and the fact that $W_{0,t_1}(\alpha) \le W_{0,t_2}(\alpha)$ proves
We can now prove
\begin{eqnarray*}
g_{t_1}(x_{j+1} :s_{-i} (\alpha))  &=&  d_j+ d(x_{t_1},x_j) +  \frac 1 {\tc_{t_1,j+1}} W_{0,t_1}(\alpha) \\
  &=&  d_j+ d(x_{t_1},x_j) +  \frac 1 {\tc_{t_1,j}}  W_{0,t_1}(\alpha) + \left(  \frac 1 {\tc_{t_1,j+1}} -   \frac 1 {\tc_{t_1,j}} \right) W_{0,t_1}(\alpha) \\
   &=&  d_j+ g_{t_1}(x_{j} :s_{-i} (\alpha)+ \left(  \frac 1 {\tc_{t_1,j+1}} -   \frac 1 {\tc_{t_1,j}} \right) W_{0,t_1}(\alpha) \\
     &\le &  d_j+ g_{t_2}(x_{j} :s_{-i} (\alpha)+ \left(  \frac 1 {\tc_{t_1,j+1}} -   \frac 1 {\tc_{t_1,j}} \right) W_{0,t_1}(\alpha)\\
   %     &\le &  d_j+ g_{t_2}(x_{j} :s_{-i} (\alpha)+ \left(  \frac 1 {\tc_{t_2,j+1}} -   \frac 1 {\tc_{t_2,j}} \right) W_{0,t_1}(\alpha) \\
             &\le &  d_j+ g_{t_2}(x_{j} :s_{-i} (\alpha)+ \left(  \frac 1 {\tc_{t_2,j+1}} -   \frac 1 {\tc_{t_2,j}} \right) W_{0,t_2}(\alpha) \\
         &=&  d_j+ d(x_{t_2},x_j) +  \frac 1 {\tc_{t_2,j}}  W_{0,t_2}(\alpha) + \left(  \frac 1 {\tc_{t_2,j+1}} -   \frac 1 {\tc_{t_2,j}} \right) W_{0,t_2}(\alpha) \\
         &=&  g_{t_1}(x_{j+1} :s_{-i} (\alpha))
\end{eqnarray*}

 Combining (a), (b) and (c) proves that if  $t_1  <  t_2 \le x_j$ then
 $$
 g_{t_1}(x_j:s_{-i} (\alpha))   \le  g_{t_2}(x_j:s_{-i} (\alpha))
 \quad \Rightarrow\quad
 g_{t_1}(x_{j+1}:s_{-i} (\alpha))   \le g_{t_2}(x_{j+1}:s_{-i} (\alpha)),$$
 which, as noted at the start of this step, proves  \Cref{eq:lcvrdown} and therefore completes Step 2.
 
 \medskip
 
  \par\noindent\underline{Step 3:} Completing the proof of Part (2).
  
 %  Combining the results of Steps 1 and 2 immediately prove that 
 %If $y' < y$  then $\lcrv(y': s_{-i} (\alpha)) \le \lcrv(y: s_{-i} (\alpha))$ completing the proof of Part 2 of the Lemma.
 Let $y' < y$ and  set $j'$ to be the unique index such that $x_{j'}< y' \le x_{j'+1}$ and $j$ to be the unique index such that $x_{j}< y \le x_{j+1}$. 
 
 From Step 1,  $\lcrv(y': s_{-i} (\alpha)) = \lcrv(x_{j'+1}: s_{-i} (\alpha))$  and $\lcrv(y: s_{-i} (\alpha)) = \lcrv(x_{j=1}: s_{-i} (\alpha)).$  
 
 Since $j' \le j$, repeated applications of Step 2 yields that 
 $\lcrv(x_{j'+1}: s_{-i} (\alpha)) \le \lcrv(x_{j+1}: s_{-i} (\alpha)).$
 
 Thus
 $$ \lcrv(y': s_{-i} (\alpha)) = \lcrv(x_{j'+1}: s_{-i} (\alpha)) \le  \lcrv(x_{j+1}: s_{-i} (\alpha)) = \lcrv(y: s_{-i} (\alpha))$$
 completing the proof of Part (2).
 
 \end{proof}


\paragraph{More about Upper Envelopes}

On an upper envelope of lines each line appears as at most one segment.
The upper envelope can then be stored as a list of lines sorted in the order in which they appear on the envelope.
In our case, the line  $g_t(x_j:s_{-i} (\alpha))$  will be represented by its index $t$ and its actual formula can  be calculated when needed.
In an upper envelope, the lines appear in order of increasing slope and only one line with a given slope may appear.
Note that the slope of  $g_t(x_j:s_{-i} (\alpha))$   is  $\frac 1 {\tc_{j,t}}$. 
For fixed $j,$   ${\tc_{j,t}}$ is {\em nondecreasing} in $t$.  Thus the $g_t(x_j:s_{-i} (\alpha))$ appear on the upper envelope in order of decreasing $t$.

For fixed $i$, our algorithms will require constructing $\lue_{i,j}$  (and $\rue_{i,j})$
 for every $j$.  Since the slopes are given in sorted order, \Cref{obs:ue} permits calculating any single one in $O(n)$ time and all of them in $O(n^2)$ time

We note without proof that, because these lower envelopes are {\em not} independent of each other, it is possible to improve this and construct all of them in a total $O(n \log n)$ time.  We do not go down that path, though, since other parts of the algorithm will require $O(n^2)$ time and improving this step would increase the complexity of the analysis without providing an overall improvement of the algorithm.


The inflection points of the upper envelope are the intersection points of two consecutive lines.
Since two lines intersect at a unique point, the inflection points of the envelope can also be calculated on the fly.
More specifically, if $f(\alpha)$ is the upper envelope  of $k$ lines the value $f(\bar \alpha)$ for any  given value $\bar \alpha$ can be found in $O(\log n)$ time.  This is done by binary searching for the inflection points to the right and  left of $\alpha$, and constructing the line segment defined by those points\footnote{except when the line segment is the half-infinite one at the beginning or end of the envelope which is defined by only one inflection point.}
and then calculating $f(\bar \alpha)$.

The algorithm will maintain the sorted list of lines as leaves in a balanced binary search tree with pointers  to successors and predecessors.  This tree can be searched and maintained, with insertions and deletions, in $O(\log n)$ time per operation.


Finally, note that because $\lue_{i,j}(\alpha)$ is a monotonically increasing  piecewise linear function of $\alpha$ with $O(n)$ inflection points, its inverse function $\lue^{-1}_{i,j}(\beta)$ exists for the range $[\lue_{i,j}(0),\infty]$ and is also  a monotonically increasing  piecewise linear function of $\alpha$ with $O(n)$ inflection points
$\lue^{-1}_{i,j}(\beta)$ with its inflection points  be constructed  in $O(n)$ time from 
%the binary tree implementation of 
$\lue_{i,j}$.


\begin{definition}
\label{def:yalpha}
Fix some scenario $s$ and  index $i$. For  $\alpha \ge 0$ define
\begin{eqnarray*}
y(\alpha) &=& x_{\OPT}\left(s_{-i}(\alpha)\right)  \\[0.1in]
\Theta(\alpha) &=& \Theta(P,y(\alpha) : s_{-i}(\alpha))\\[0.1in]
\lcrv(\alpha) &=& \lcrv\left(y(\alpha) :  s_{-i}(\alpha))\right)\\[0.1in]
\rcrv(\alpha) &=& \rcrv\left(y(\alpha) :  s_{-i}(\alpha))\right)
\end{eqnarray*}
\end{definition}
Consider $y(0) = x_\OPT\left(s_{-i}(0)\right).$ 
    Intuitively, as $\alpha$ increases,  $y(\alpha)$ either   stays in the same location or moves towards $x_i$, which is starting with more and more flow.  When $\alpha$ gets large enough,  $y(\alpha) = x_i$.  After that, $y(\alpha)$ will remain on $x_i.$
    This intuition is encapsulated in the following lemma which also explores how the critical vertices can change.
\begin{lemma}
\label{lem:yalpha}
Fix $s,i$ as in \Cref{def:yalpha}. Then 

\begin{enumerate}
\item $\Theta(\alpha)$ is a   non-decreasing  continuous function of  $\alpha$. %  with $O(n)$ critical points
\item There exists $\bar\alpha$ such that
	\begin{itemize}
		\item $\bar\alpha = \min\left\{ \alpha \ge 0 \,:\,  \Theta(\alpha)= \Theta\left(P,x_i:s_{-i}(0)\right)\right\}= \min\left\{ \alpha \ge 0 \,:\,  y(\alpha) =x_i  \right\}.$
			\item $\forall  \alpha \ge \bar \alpha, $   $y(\alpha) =x_i$  and $\Theta(\alpha) = \Theta\left(P,x_i:s_{-i}(0)\right).$
	\end{itemize}
\item (a)  If $y(0) > x_i$, then $y(\alpha)$ is a  non-increasing function of $\alpha$ satisfying $\forall \alpha,\,  y(\alpha) \ge x_i.$\\
(b) If $y(0) < x_i$, then $y(\alpha)$ is a  non-decreasing function of $\alpha$  satisfying $\forall \alpha,\,  y(\alpha) \le x_i.$\\
(c) If $y(0) = x_i$, then $y(\alpha) \equiv x_i$.\\
\item $\lcrv(\alpha)$ is a non-increasing function of $\alpha$.
\end{enumerate}


\end{lemma}

\begin{proof}
%First note that,  by construction {\color{red}(****NEEDS MORE****)}  $\Theta(\alpha)$ is a  continuous functions of $\alpha$. 
\ 

\par\noindent\underline{Step 1:}   Let $ \alpha < \alpha'$.
We first show that 
 $\Theta(\alpha) \le  \Theta(\alpha')$.



From \Cref{lem:env}, for fixed $y,$  $\Theta (P,y: s_{-i} (\alpha))$ is, as a function of $\alpha,$ an  upper envelopes of a set of lines, all with nonnegative slope.  Thus
$$
 \Theta\left(P,y:s_{-i}(\alpha)\right)  \le   \Theta\left(P,y:s_{-i}(\alpha')\right) 
$$ 
so 
$$\Theta(\alpha) =  \min_{y\in P} \Theta\left(P,y:s_{-i}(\alpha)\right) \le   \min_{y \in P} \Theta\left(P,y:s_{-i}(\alpha')\right)  = \Theta(\alpha').$$



\par\noindent\underline{Step 2:} We now prove that $\Theta(\alpha)$ is continuous, concluding the proof of point (1).\\[0.05in]

 Let $ \alpha < \alpha'$  Recall that for any $y,$ 
$\Theta\left(P,y:s_{-i}(\alpha\right))$ is a piecewise linear function with slopes $\le \tilde c =  \max_j 1/c_j.$  Thus, for any $y,$
$$\Theta\left(P,y:s_{-i}(\alpha'\right)) - \Theta\left(P,y:s_{-i}(\alpha\right)) \le \tilde c (\alpha' - \alpha).$$
The continuity of $\Theta(\alpha)$ follows from the fact that
%\begin{eqnarray*} 
%\Theta\left(P,y(\alpha):s_{-i}(\alpha\right))   &=& \Theta(\alpha)\\	
%								 &\le&  \Theta(\alpha')\\
%								 &=&\Theta\left(P,y(\alpha'):s_{-i}(\alpha'\right)) \\
%								 &=&\Theta\left(P,y(\alpha):s_{-i}(\alpha'\right)) \\
%								&\le&\Theta\left(P,y(\alpha):s_{-i}(\alpha\right))  + \tilde c (\alpha' - \alpha).
%\end{eqnarray*}
\begin{eqnarray*} 
 \Theta(\alpha)&\le&  \Theta(\alpha')\\
%&=&\Theta\left(P,y(\alpha'):s_{-i}(\alpha'\right)) \\
 &\le&\Theta\left(P,y(\alpha):s_{-i}(\alpha'\right)) \\
&\le&\Theta\left(P,y(\alpha):s_{-i}(\alpha\right))  + \tilde c (\alpha' - \alpha)\\
&=& \Theta(\alpha))+ \tilde c (\alpha' - \alpha).
\end{eqnarray*}

\medskip

\par\noindent\underline{Step 3:}  Proving point (2).\\[0.1in]


%First note that for  $\alpha >0,$  
%		$ \Theta(\alpha)= \Theta\left(P,x_i:s_{-i}(0)\right\}$ if and only if  
%		$  y(\alpha) =x_i.$
		
		
		First  note that, if $y \not=x_i$, then all flow from $x_i$ to $y$ must pass through at least part of the edge $(x_{i-1},x_i)$ with capacity $c_{i-1}$ or
 $(x_{i},x_{i+1})$ with capacity $c_{i}$.  Thus, if $y(\alpha) \not= x_i$ then $\theta(\alpha) \ge \frac {\alpha} {\max(c_{i-1},c_i)}$ which will approach $\infty$ as $\alpha \uparrow \infty.$   If $y(\alpha)=x_i$ then $\Theta(\alpha) = \Theta\left(P, x_i:s_{-i}(0)\right),$ independent of $\alpha$. Thus there exists some $\alpha'$ such that $y(\alpha') = x_i$ and thus  $\Theta(\alpha') = \Theta\left(P, x_i:s_{-i}(0)\right).$
 
 The continuity of $\Theta(\alpha)$  proves the existence of 
 $$\tilde \alpha = \min\left\{ \alpha \ge 0 \,:\,  \Theta(\alpha)= \Theta\left(P,x_i:s_{-i}(0)\right)\right\}.$$

 
 From Point (1), if $\alpha > \tilde \alpha$ ,  $\Theta(\alpha)   \ge \Theta(\tilde \alpha).$  This imples
 $$\Theta(\alpha)   \ge \Theta(\tilde \alpha) = \Theta\left(P,x_i:s_{-i}(0)\right)= \Theta\left(P,x_i:s_{-i}(\alpha)\right).
 $$
 This immediately implies that 
 $\forall  \alpha \ge \tilde \alpha, $   $y(\alpha) =x_i$  and $\Theta(\alpha) = \Theta_L\left(P,x_i:s_{-i}(0)\right).$
 
Finally, note that if $\alpha'' <  \tilde \alpha$ then $y(\alpha') \not= x_i$.  This is because if $y(\alpha') = x_i$, then
$\Theta(\alpha') = \Theta\left(P,x_i:s_{-i}(0)\right)$ which, by the definition of $\tilde \alpha$ implies $\alpha' \ge \tilde \alpha.$
Thus
$$\min\left\{ \alpha \ge 0 \,:\,  \Theta(\alpha)= \Theta\left(P,x_i:s_{-i}(0)\right)\right\}= \min\left\{ \alpha \ge 0 \,:\,  y(\alpha) =x_i  \right\}.$$

\medskip


\par\noindent\underline{Step 4:}   

Consider  $y(0).$ If $y(0) = x_i$ then from point (2),  $\forall \alpha \ge 0,$   $y(\alpha) = x_i$ and point 3 is trivially obvious.

We will now prove Point (3) by showing that
\begin{equation}
\label{eq:ya1}
 \mbox{If } y(\alpha) > x_i \quad \mbox{and} \quad  \alpha' > \alpha \quad \mbox{  then}   \quad x_i \le y(\alpha') \le y (\alpha)
 \end{equation}
and 
\begin{equation}
\label{eq:ya2}
\mbox{If } y(\alpha) < x_i \quad \mbox{and} \quad  \alpha' > \alpha \quad \mbox{  then}   \quad y(\alpha) \ge y (\alpha') \ge x_i.
\end{equation}


We actually prove  a more technical result that will imply \Cref{eq:ya1,eq:ya2} This is:
 \begin{equation}
\label{eq:ya3a}
\mbox{If $x_i \le \bar y \le y'$  and }\ \Theta(P,\bar y:s_{-i}(\alpha)) \le  \Theta(P,y':s_{-i}(\alpha))
\quad \Rightarrow \quad \forall \alpha' > \alpha,\ \ \Theta(P,\bar y:s_{-i}(\alpha')) \le \Theta(P,y':s_{-i}(\alpha'))
\end{equation}
and
\begin{equation}
\label{eq:ya3b}
\mbox{If  $y' \le \bar y \le x_i$  and }\ \Theta(P,\bar y:s_{-i}(\alpha)) \le \Theta(P,y':s_{-i}(\alpha))
\quad \Rightarrow \quad \forall \alpha' > \alpha,\ \ \Theta(P,\bar y:s_{-i}(\alpha')) \le  \Theta(P,y':s_{-i}(\alpha')).
\end{equation}

To see that \Cref{eq:ya3a,eq:ya3b} imply \Cref{eq:ya1} set $\bar y = y(\alpha)\ge x_i$ and suppose $y' > y(\alpha).$ Then 
\Cref{eq:ya3a} implies that for $\alpha' > \alpha,$ $ \Theta(P,\bar y(\alpha):s_{-i}(\alpha')) \le \Theta(P,y':s_{-i}(\alpha')).$ Since this is true for all $y' > y(\alpha)$,  this implies  $y(\alpha') \le y(\alpha).$

Next suppose that $y(\alpha')  < x_i$.  Because $\Theta\left(P,x:s_{-i}(\alpha)\right)$ is a unimodal function in $x$ with unique minimum at $x = y(\alpha) > x_i$ we have that 
$$\Theta\left(P,y(\alpha) :s_{-i}(\alpha)\right)  < \Theta\left(P,x_i :s_{-i}(\alpha)\right) <  \Theta\left(P,y':s_{-i}(\alpha)\right).$$
Setting $\bar y = x_i$ and applying \Cref{eq:ya3b} implies that $\Theta\left(P,x_i :s_{-i}(\alpha)\right) \le  \Theta\left(P,y':s_{-i}(\alpha')\right)$

But this contradicts the definition of $y(\alpha')$ which, if $y(\alpha') \not=x_i,$  requires  
$\Theta\left(P,x_i :s_{-i}(\alpha)\right) >  \Theta\left(P,y':s_{-i}(\alpha')\right)$. We have thus just proven that \Cref{eq:ya3a,eq:ya3b} imply \Cref{eq:ya1}.

\medskip

It now remains to prove \Cref{eq:ya3a}.  The proof of \Cref{eq:ya3b} is symmetric and will be omitted.


\medskip

We assume that  $x_i \le \bar y \le y'$  and $\Theta(P,\bar y:s_{-i}(\alpha)) \le  \Theta(P,y':s_{-i}(\alpha))$.

If  \Cref{eq:ya3a} is incorrect there exists $\alpha' > \alpha$ such that 
\begin{equation}
\label{eq:barprimealpha}
\Theta(P,\bar y:s_{-i}(\alpha')) > \Theta(P,y':s_{-i}(\alpha')).
\end{equation}

By monotonicity
$$\forall \beta \ge 0,\quad \Theta_L(P,\bar y:s_{-i}(\beta)) \le \Theta_L(P,y':s_{-i}(\beta))$$
and, in particular, 
$$ \Theta_L(P,\bar y:s_{-i}(\alpha')) \le \Theta_L(P,y':s_{-i}(\alpha')).$$
Thus, from \Cref{eq:barprimealpha},
\begin{eqnarray*}
\Theta_R(P,\bar y:s_{-i}(\alpha))  &=& \Theta_R(P,\bar y:s_{-i}(\alpha'))  \\
&=& \Theta(P,\bar y:s_{-i}(\alpha'))\\
&>& \Theta(P, y':s_{-i}(\alpha')).
\end{eqnarray*}
In particular, this implies
\begin{eqnarray*}
\Theta_R(P,\bar y:s_{-i}(\alpha)) 
&>& \Theta(P, y':s_{-i}(\alpha'))\\
&\ge&  \Theta_R(P,y':s_{-i}(\alpha'))\\
&=&  \Theta_R(P,y':s_{-i}(\alpha))
\end{eqnarray*}
and
\begin{eqnarray*}
\Theta_R(P,\bar y:s_{-i}(\alpha)) 
&>& \Theta(P, y':s_{-i}(\alpha'))\\
&\ge&  \Theta_L(P,y':s_{-i}(\alpha'))\\
&>&  \Theta_L(P,y':s_{-i}(\alpha)).
\end{eqnarray*}
This implies
\begin{eqnarray*}
\Theta(P,\bar y:s_{-i}(\alpha)) 
&\ge& \Theta_R(P,\bar y:s_{-i}(\alpha)) \\
&>& \max\left(  \Theta_L(P, y':s_{-i}(\alpha)),\, \Theta_R(P, y':s_{-i}(\alpha))\right)\\
&=&  \Theta(P,y':s_{-i}(\alpha)).
\end{eqnarray*}
contradicting the original assumption.

This proves  \Cref{eq:ya3a}.







\par\noindent\underline{Step 5:}  Let $\alpha < \alpha'$.  From (1) $y(\alpha') \le y(\alpha).$  Thus, from \Cref{lem:crv change},
\begin{eqnarray*}
\lcrv(\alpha') &=& \lcrv\left(y(\alpha') :  s_{-i}(\alpha'))\right)\\
			&\le& \lcrv\left(y(\alpha) :  s_{-i}(\alpha'))\right)\\
			&\le& \lcrv\left(y(\alpha) :  s_{-i}(\alpha))\right)\\
			&=&\lcrv(\alpha).
\end{eqnarray*}
\end{proof}


\begin{definition}
Fix $s,i$ as in \Cref{def:yalpha} and, for $k \ge i$ define $z_k$ and for $k>i$ define $\bar z_k$ as 
\begin{eqnarray*}
z_k &=& \Theta_R(P,x_k :s_{-i} (\alpha))\\
\bar z_k &=& \Theta_R^-(P,x_k :s_{-i} (\alpha)) = \Theta_R(P,x_{k-1}:s_{-i} (\alpha)) - d_{k-1} = z_{k-1} -d_{k-1}
\end{eqnarray*}
Note that since $k \ge i$,  the $z_k$ and thus the $\bar z_k$ are  constants independent  of $\alpha$.  Also
$$z_i    > \bar z_{i+1} \ge  z_{i+1} > \bar  z_{i+2} \ge  z_{i+2} \cdots >\bar z_{n-1} \ge  z_{n-1} > \bar z_n \ge z_n .$$
\end{definition}




\begin{lemma}
\label{lem:yalpha5p}
Fix $s,i$, $y(\alpha)$ and  $\Theta(\alpha)$ as in \Cref{def:yalpha}. 


If $y(0) = x_i$,  then 
$\forall \alpha \ge 0$,  $y(\alpha) = x_i$ and
$\Theta(\alpha) = \Theta(P,x_i, s_{-1}(0)).$

\medskip



 If $y(0) > x_i$, then
 \begin{enumerate}
 \item For $\alpha \ge 0,$ 
		\begin{equation}
		\label{eq:bar6p}
		\begin{array}{lccccc}
		(i)  & \quad &				           & z_i \le \Theta(\alpha) 			   & \quad \Leftrightarrow \quad &  y(\alpha) =  x_i,\\
		(ii)  & \quad & \mbox{For $k \ge i$,}\  & \bar z_{k+1} <\Theta(\alpha) <  z_k & \quad \Leftrightarrow \quad & x_k < y(\alpha) < x_{k+1},\\
		(iii) & \quad &  \mbox{For $k > i$,}\  & z_k \le \Theta(\alpha)  \le  \bar z_{k}   & \quad \Leftrightarrow \quad & y(\alpha)=x_k,\\
		(iv)  & \quad &  					   &  \Theta(\alpha)  	 \le z_n		    & \quad \Leftrightarrow \quad & y(\alpha)=x_n.\
		\end{array}
		\end{equation}
\item  		In the different cases $\Theta(\alpha)$ is defined, respectively, by
		\begin{equation}
		\label{eq:bar7p}
			\begin{array}{lcccc}
		(i)  & \quad 				           &\Theta(\alpha) &=&   \Theta(P,x_i:s_{-i}(\alpha))\\
		(ii)  & \quad 				           &\Theta(\alpha) &=&   z_k - (y(\alpha)-x_k)\\
		(iiii) & \quad  				           &\Theta(\alpha) &=&  \Theta(P,x_k:s_{-i}(\alpha))\\
		(iv)  & \quad  					     &\Theta(\alpha) &=&   	\Theta(P,x_n:s_{-i}(\alpha))
		\end{array}	
		\end{equation}
       \item  $y(\alpha)$ is  a nonincreasing continuous function of $\alpha.$       
\end{enumerate}
\end{lemma}
\begin{proof}
From \Cref{lem:yalpha}, if $y(0) = x_i$ then $\forall \alpha \ge 0$,  $y(\alpha) = x_i$, Case (i) always holds and the lemma is trivially correct.

We therefore assume $y(0) > x_i.$ Again, from \Cref{lem:yalpha}, we know that, $\forall \alpha > 0,$  $y(\alpha) \ge x_i.$  Now consider the dynamics of $y(\alpha)$ and $\Theta(\alpha).$


\medskip

First consider case (ii).  If $y(\alpha) = y  \in (x_k,x_{k+1})$  for some  $k\ge i$ then, from \Cref{lem:opt equal} and the fact that 
$y =x_{\OPT}\left(s_{-i}(\alpha)\right) $

\begin{eqnarray*}
\Theta(\alpha) &=& \Theta_L(P,y :s_{-i} (\alpha)) \\
&=& \Theta_R(P,y :s_{-i} (\alpha)) \\
&=& \Theta_R(P, x_k: s_{-i}  (\alpha)) -(y-x_k) \\
&=& z_k - (y-x_k).
\end{eqnarray*}
This implies, for all $k \ge i,$
\begin{equation}
\label{eq:yalpha4p}
\mbox{If}   \quad x_k< y(\alpha) < x_{k+1}
\quad \quad \Rightarrow \quad \quad 
z_k > \Theta(\alpha) > z_k-d_k = \bar z_{k+1} \quad   \wedge \quad y(\alpha) = z_k +x_k - \Theta(\alpha).
\end{equation}


Now suppose that $\Theta(\alpha) = z'$ where  $z_k> z' > \bar z_{k+1}$ for some $k \ge i.$
Set $y' = x_k + (z_k - z').$  Then  $y' > x_k$  and 
$$y' = x_k + (z_k - z') < x_k + (z_k - \bar z_{k+1}) = x_k + d_k  = x_{k+1}$$ so
$x_k< y' < x_{k+1}$.
% Let $y'$ be such that $x_k< y' < x_{k+1}$ and  $z' = z_k - (y'-x_k).$ 
By construction
$$\Theta_R\left(P,y':s_{-i}(\alpha)\right) \bigr) = z_k - (y'-x_k) = z' = \Theta(\alpha) .$$

Observe that
$y(\alpha) \ge y'$ since if $ y(\alpha) < y'$
$$\Theta(\alpha)  \ge \Theta_R(P, y(\alpha):s_{-i} (\alpha)) > \Theta_R(P, y':s_{-i} (\alpha)) = \Theta(\alpha),
$$
leading to a contradiction.
Observe further that $y(\alpha) \ge y'$  implies
$$\Theta(\alpha) \ge \Theta_L(P, y(\alpha):s_{-i} (\alpha))\ge \Theta_L(P, y':s_{-i} (\alpha)).$$
Thus  
\begin{eqnarray*}
\Theta(P, y':s_{-i} (\alpha)) &=&
\max \bigl( \Theta_L\left(P,y':s_{-i}(\alpha)\right),\, \Theta_R\left(P,y':s_{-i}(\alpha)\right) \bigr)\\
				&\le& \max \bigl( \Theta(\alpha),\, \Theta(\alpha) \bigr) = \Theta(\alpha).
\end{eqnarray*}
\medskip
Thus by the definition of $\Theta(\alpha)$, $\Theta(P, y':s_{-i} (\alpha)) = \Theta(\alpha)$.
From the definition of $y(\alpha)$ this implies $y(\alpha) \le y'$ and thus $y(\alpha) = y'$.

This shows
\begin{equation}
\label{eq:yalpha5p}
\mbox{If}   
\quad 
z_k >\Theta(\alpha) >  \bar z_{k+1}
\quad \Rightarrow \quad
x_k< y(\alpha) < x_{k+1}
\end{equation}
Combined with \Cref{eq:yalpha4p} this implies
\begin{equation}
\label{eq:yalpha6p} 
z_k> \Theta(\alpha) >  \bar z_{k+1}
\quad \Leftrightarrow \quad
x_k < y(\alpha)  = z_k+ x_k - \Theta(\alpha) < x_{k+1}.
\end{equation}
%Under the assumption that $\bar \alpha = \beta,$
 This proves case (ii) of \Cref{eq:bar6p,eq:bar7p}.

 \Cref{lem:yalpha}  says that $\Theta(\alpha)$ is a continuous nondecreasing function.   Combined with the fact that $y(\alpha)$ is a nonincreasing function of $\alpha$ this imediately implies
cases (i),  (iii) and (iv) of \Cref{eq:bar6p,eq:bar7p}.  This in turn implies the fact that $y(\alpha)$ is continuous.



\end{proof}

\begin{lemma}
\label{lem:yalpha5pp} 
Fix $s,i$  and  define $y(\alpha)$,  $\Theta(\alpha)$ as in \Cref{def:yalpha}.  Assume $y(0) \ge x_i$  and 
for  $i <k \le  n$ define
$$\alpha_k = \mbox{unique value $\alpha$ such that } \Theta_L(P,x_{k+1}:s_{-i}(\alpha)) = z_k+ d_k
$$
and  for  $i < k \le  n$
define
$$\bar \alpha_k = \mbox{unique value $\alpha$ such that } \Theta_L(P,x_{k}:s_{-i}(\alpha)) = \bar z_k = z_{k-1}-d_k.
$$
(Note that it while it is technically  possible that some of the $\alpha_k,\bar \alpha_k$ are negative these values will never be used.)

Then

		\begin{equation}
		\label{eq:bar10p}
		\begin{array}{cccccccc}
						           &  \alpha \le \alpha_n 			   & \quad \Rightarrow \quad &  y(\alpha) = x_n & \mbox{ and } &  \Theta(\alpha) &=& \Theta(P,x_n:s_{-i}(\alpha)),\\
		  \mbox{If, for $i < k \le n$,}\  & \alpha_k \le \alpha  \le  \bar \alpha_{k}   & \quad \Rightarrow \quad &  y(\alpha) = x_k & \mbox{ and } & \Theta(\alpha) &=& \Theta(P,x_k:s_{-i}(\alpha)),\\
		 \mbox{If, for $i \le k < n$,}\  & \bar \alpha_{k+1} <\alpha < \alpha_k & \quad \Rightarrow \quad &  y(\alpha) = f_k(\alpha) & \mbox{ and } &\Theta(\alpha) &=&z_k - (y(\alpha)-x_k),\\
		  					   &  \alpha_i \le \alpha  		    & \quad \Rightarrow \quad &   y(\alpha) = x_i & \mbox{ and } &  \Theta(\alpha) &=& \Theta(P,x_i:s_{-i}(\alpha)),
		\end{array}
		\end{equation}
		where 
$$f_k(\alpha) =\frac 1 2 ( z_k - \Theta_L(P, x_{k+1}:s_{-i}(\alpha)) + d_k + 2 x_k).$$
Furthermore $y(\alpha)$ and $\Theta(\alpha)$ are piecewise linear functions with $O(n)$ inflection points that can be constructed in total time
% $O(n \log n)$.
$O(n^2).$
\end{lemma}
\begin{proof}
\ 

\par\noindent\underline{Step 1:}  %Constructing the $z_k$ and $\bar z_k$ in $O(n \log n)$ time.
Constructing the $z_k$ and $\bar z_k$ in $O(n^2)$ time.

%Using \Cref{lem:UE} iteratively construct  $\rue_{i,k}(\alpha)$ for $k=n,n-1,\ldots,j$.  This can be done in $O(\log n)$ time for each $k.$
% At the time  $\rue_{i,k}(\alpha)$ is built,  $z_k$ can be constructed in $O(\log n)$ time for a total of $O(n \log n)$ time.
% Once the $z_k$ are constructed, the $\bar z_k$ can be constructed in $O(n)$ total time.
 
Construct  $\rue_{i,k}(\alpha)$ for $k=n,n-1,\ldots,j$.  Each one can be constructed in $O(n)$ time.
At the time  $\rue_{i,k}(\alpha)$ is built,  $z_k$ can be constructed in $O(n)$ futher time.
Once the $z_k$ are constructed, the $\bar z_k$ can be constructed in $O(n)$ total time.
 In total, this process requires $O(n^2)$ time.
\medskip


 \par\noindent\underline{Step 2:}  Constructing the $\alpha_k$ and ${\bar \alpha}_k$ in $O(n \log n)$ time.

%Using \Cref{lem:UE} iteratively construct  $\lue_{i,k}(\alpha)$ for $k=j,j+1,\ldots,n$.  This can be done in $O(\log n)$ time for each $k.$
% At the time  $\lue_{i,k}(\alpha)$ is built,   ${\bar \alpha}_{k-1}$   and $\alpha_k$   can each be found in $O(\log n)$ time for a total of $O(n \log n)$ time.

Construct  $\lue_{i,k}(\alpha)$ for $k=j,j+1,\ldots,n$.  Each one can be constructed in $O(n)$ time.
 At the time  $\lue_{i,k}(\alpha)$ is built,   ${\bar \alpha}_{k-1}$   and $\alpha_k$   can each be constructed in $O(n)$ time for a total of $O(n^2)$ time.

%
% 
% 
% \medskip
% \par\noindent\underline{Step 3:}
%Use the algorithm from  \cite {BGYKK2017}  to  find %$x^{**}=x_{\OPT}\left(s_{-i}( w_i^+)\right)$ 
% $x^{*}=x_{\OPT}\left(s_{-i}( w_i^-)\right)$  
%in $O(n\log n)$ time\footnote{Technically, this  could also be done using \Cref{lem:UE} and the observations following it.}.

% \medskip
% \par\noindent\underline{Step 3:}   If $x^* \le x_j$ then Case 1 from \Cref{lem:yalpha5} states that
% \Cref{eq:bar11} is correct.
% 
% Furthermore
% $$ \Theta(\alpha) = \Theta(P,x_j:s_{-i}(\alpha)) = \min\Bigl( \lue_{i,j}(\alpha),\, z_j  \Bigr)$$
% which can be built in $O(n \log n)$ time from \Cref{lem:UE} . The fact that it has $O(n)$ inflection points follows from the definition of $ \lue_{i,j}(\alpha).$



 \medskip
 \par\noindent\underline{Step 3:}   \Cref{lem:yalpha5p} 
  immediately implies that \Cref{eq:bar10p} is correct with the exception of the third line
 $$\mbox{If, for $i \le k < n$,}\   \alpha_{k+1} <\alpha < \alpha_k \quad \Rightarrow \quad   y(\alpha) = f_k(\alpha)   \mbox{ and } \bar \Theta(\alpha) = z_k - (y(\alpha)-x_k).$$
 To see why this line is correct note that  % in this case  $y(\alpha) = y(\alpha)$ and  \Theta(\alpha) = \Theta(\alpha)$.
 From 2(ii)  of   \Cref{lem:yalpha5p} and the definition of $\bar \alpha_{k}$ and $\alpha_k$
\begin{eqnarray*}
{\bar \alpha}_{k+1} < \alpha<  \alpha_k & \quad \Leftrightarrow \quad &   \bar z_{k+1} <\Theta(\alpha) <  z_k \\
   & \quad \Leftrightarrow \quad & x_k < y(\alpha) < x_{k+1}.
\end{eqnarray*}

If  $x_k < y(\alpha) \le x_{k+1}$  set 
$\delta' = y(\alpha) - x_k.$ 
From \Cref{cor:smooth evac}, we know this only happens if 
$$ \Theta(\alpha) =  \Theta(P,y(\alpha):s_{-i}(\alpha)) = \Theta_L(P,y(\alpha):s_{-i}(\alpha)) = \Theta_R(P,y(\alpha):s_{-i}(\alpha)).$$
Thus
\begin{eqnarray*}
\Theta_L(P,x_{k+1}:s_{-i}(\alpha))  - (d_j-\delta')
&=& \Theta_L(P,y(\alpha):s_{-i}(\alpha)) \\  
&=& \Theta_R(P,y(\alpha):s_{-i}(\alpha))\\
&=& \Theta_R(P,x_k:s_{-i}(\alpha)) - \delta'\\
&=& z_k - \delta'.
\end{eqnarray*}
 So
 $$2 (y(\alpha) - x_k) = 2 \delta' = z_k - \Theta_L(P, x_{k+1}:s_{-i}(\alpha)) + d_j.
 $$
This immediately implies that 
$$ y(\alpha) = \frac 1 2 ( z_k - \Theta_L(P, x_{k+1}:s_{-i}(\alpha)) + d_k + 2 x_k).$$
and
\begin{eqnarray*}
%\bar \Theta(\alpha)  =
 \Theta(\alpha) &=& z_k - \delta' \\
                     &= & z_k - (y(\alpha) - x_k)\\
                     &=&  \frac 1 2  (z_k +  d_k)   + \frac 1 2  \Theta_L(P, x_{k+1}:s_{-i}(\alpha)).
 \end{eqnarray*}                    
This completes the proof of \Cref{eq:bar10p} which immediately shows that $\bar y(\alpha)$ and $\bar \Theta(\alpha)$ are piecewise linear functions.






 \medskip
 \par\noindent\underline{Step 5:} 
 It is now easy to construct  $y(\alpha)$ and $\Theta(\alpha)$.  For each case of \Cref{eq:bar10p}  identify the appropriate interval of $\alpha$,
   and then pull off the part of the corresponding upper envelope that confirms to this interval. 

More specifically, first assume Case (ii), 
$\alpha \in\left( \alpha_{k+1}, \alpha_k \right)$ for some $k$. For these $\alpha$ 
\begin{eqnarray*}
\Theta(\alpha) &=&    \Theta_L(P, y(\alpha):s_{-i}(\alpha)) = \frac 1 2  (z_k +  d_k)   + \frac 1 2  \Theta_L(P, x_{k+1}:s_{-i}(\alpha)),\\
y(\alpha) &=& \frac 1 2 ( z_k - \Theta_L(P, x_{k+1}:s_{-i}(\alpha)) + d_k + 2 x_k).
\end{eqnarray*}
The only possible inflection points for $\Theta(\alpha)$  {\em within} these ranges are the inflection points of  $\Theta_L(P, x_{k+1}:s_{-i}(\alpha))$ within these ranges. At these inflection points $ \lcrv(\alpha)=  \lcrv\left(y(\alpha) :  s_{-i}(\alpha))\right)$ decreases.  
 From \Cref{lem:yalpha} part 4,  $ \lcrv(\alpha)$ is a non-increasing function of $\alpha$ so it can only decrease $n-1$ times over all possible $k.$ 
 
 From the continuity of $y(\alpha)$ these and the points $x_k$ are the only possible inflection points for $y(\alpha)$ so $y(\alpha)$ is a piecewise linear function with at most$ O(n)$ inflection points.
 
 
 \medskip
 
 Now consider  case (ii), i.e., 
 for $ i <  k \le$,\  
 $\alpha \in \left[ \alpha_k,  \bar \alpha_{k} \right]$ where we set
 $\alpha_0 =0$ and $\alpha_n = \infty.$ 
 In these cases
\begin{eqnarray*}
  \Theta(\alpha) &=& \Theta(P,x_k:s_{-i}(\alpha))\\
  			     &=&  \max\left( \Theta_L(P,x_k:s_{-i}(\alpha)),\,  \Theta_R(P,x_k:s_{-i}(\alpha))\right)\\
   			     &=&  \max\left( \Theta_L(P,x_k:s_{-i}(\alpha)),\,  z_k\right)
 \end{eqnarray*}
 Next note that $ \Theta_L(P,x_k:s_{-i}(\alpha))$ is  a monotonically increasing function so, for fixed $k$,  $\Theta(\alpha)$  starts with (possibly) the constant value $z_k$, and then switches, at some point to being $ \Theta_L(P,x_k:s_{-i}(\alpha)) =  \Theta_L(P,y(\alpha):s_{-i}(\alpha)).$  The total number of inflection points for a fixed $k$ is then at most $1+$ the number of inflection points for $ \Theta_L(P,y(\alpha):s_{-i}(\alpha))$ when $\alpha \in \left[ \alpha_k,  \bar \alpha_{k} \right]$ .
 Again, from  \Cref{lem:yalpha} part 4,  over {\em all} $\alpha$ and thus over all $k,$ the total number of inflection points of   $ \Theta_L(P,y(\alpha):s_{-i}(\alpha))$  is $O(n)$ so the total number of inflection points that occur in Case (ii) is $O(n).$
 
 
 Next assume Case (i), that $ \alpha \le \alpha_n $		so 	   $ y(\alpha) = x_n$
 and
$$
  \Theta(\alpha) =\Theta(P,x_n:s_{-i}(\alpha)).
  $$
 From \Cref{lem:env} this function has at most $O(n)$ inflection points.
 
 
Finally, in Case (iv)
$\alpha_i \le \alpha$ implies 		    $ y(\alpha) = x_i $
and 
$$ \Theta(\alpha) =  \Theta(P,x_i:s_{-i}(\alpha)) =  \Theta(P,x_i:s_{-i}(0))$$
which is a constant so it contains no inflection points.

Combining all of the cases above shows that $ \Theta(\alpha)$ has $O(n)$ inflection points.




\end{proof}


\begin{lemma}
\label{lem:yalpha5}
Fix $s,i$. and  define $y(\alpha)$,  $\Theta(\alpha)$ as in \Cref{def:yalpha}.  Assume $y(0) \ge x_i$
Set  $I =  [x_j,x_t]$ with $i \le j \le t$ and define
\begin{eqnarray*}
\bar y(\alpha) &=& \argmin_{y \in I}  \Theta(P, y:s_{-i} (\alpha)), \\[0.1in]
\bar \Theta(\alpha) &=& \Theta(P,\bar y(\alpha) : s_{-i}(\alpha)).
\end{eqnarray*}
Then
$$
\bar y(\alpha) =
\left\{
\begin{array}{ll}
x_t & \mbox{if $\alpha \le \alpha_t$}\\
y(\alpha) &   \mbox{if $\alpha_t \le \alpha \le \alpha_j$}\\
x_j & \mbox{if $\alpha_j \le \alpha$}.\
\end{array}
\right.
\quad \mbox{and}  \quad
\bar \Theta(\alpha) =
\left\{
\begin{array}{ll}
 \Theta(P, x_t : s_{-i}(\alpha)) & \mbox{if $\alpha \le \alpha_t$}\\
\Theta(\alpha) &   \mbox{if $\alpha_t \le \alpha \le \alpha_j$}\\
 \Theta(P, x_j : s_{-i}(\alpha))& \mbox{if $\alpha_j \le \alpha$}.\
\end{array}
\right.
.
$$
Furthermore,  $\bar y(\alpha),$  and $\bar \Theta(\alpha)$ are piecewise linear, respectively, non-increasing and increasing, functions with $O(n)$ inflection points that can be constructed in $O(n^2)$ time.
\end{lemma}
\begin{proof}
Note that if $\alpha_t \le \alpha \le \alpha_j$ then,  from \Cref {lem:yalpha5pp},
$x_t \le y(\alpha) \le x_j$ so 
 trivially $\bar y(\alpha)  = y(\alpha)$ since $y(\alpha)$ is minimal over the entire path and not just $I.$


If  $\alpha_j  < \alpha,$   then, from  \Cref {lem:yalpha5pp}, $y(\alpha) \le x_j.$
From  \Cref{obs: unimodal}, $\Theta(P,y,(s_{-i}(\alpha))$ is a unimodal function of $y$ with minimum at 
$y(\alpha)$.  
Thus
$$\forall y \in I,\,  \Theta(P,x_j,(s_{-i}(\alpha)) \le \Theta(P,y,(s_{-i}(\alpha))$$
and  $\bar y(\alpha) = x_j.$

Similarly, if $\alpha <\alpha_t,$ then,   from  \Cref {lem:yalpha5pp}, $y(\alpha) \ge x_t.$ Again, since 
$\Theta(P,y,(s_{-i}(\alpha))$ is a unimodal function of $y$ with minimum at 
$y(\alpha)$,
$$\forall y \in I,\,  \Theta(P,x_t,(s_{-i}(\alpha)) \le \Theta(P,y,(s_{-i}(\alpha))$$
and  $\bar y(\alpha) = x_t.$

The rest of the Lemma's statements follow immediately from the properties of $\Theta(\alpha)$,  $y(\alpha)$ and the functios
$\Theta(P, x_j : s_{-i}(\alpha))$  and $\Theta(P, x_t : s_{-i}(\alpha))$

\end{proof}

\subsection{Efficient Computation of $G(x)$ and $H(x)$}

\begin{lemma}
\label{lem:Gj}
Fix $x$  Then 
\begin{enumerate}
\item For any $j,$   $G_{j}(x)$ can be calculated in $O(n^2)$ time.
\item For any $i,$   $H_{j}(x)$ can be calculated in $O(n ^2)$ time.
\end{enumerate}
\end{lemma}
\begin{proof}
Set $s = s_{j,j}(0,0).$ Recall that
\begin{eqnarray*}
G_{j} (x)& =&\max_{ s \in S_{j,j}} \left\{ g_j(x:s) - \min_{y \ge x_j} \Theta(P,y:s)  \right\}\\
&=&  \max_{\alpha \in \left[ w_j^-,\,w_j^+\right]} \left\{ g_j(x:s_{-j}(\alpha)) - \min_{y \ge x_j} \Theta(P,y:s_{-j}(\alpha))  \right\}\\
\end{eqnarray*}
From \Cref{lem:yalpha5},   $\min_{y \ge x_j} \Theta(P,y:s_{-i}(\alpha))$ is a piecewise linear function with $O(n)$ inflection points (on the nonnegative half line $\alpha \ge 0$) that can be constructed in $O(n^2)$ time.

 $g_j(x:s_{-i}(\alpha)) - \min_{y \ge x_j} \Theta(P,y:s_{-i}(\alpha))$ is then also a  piecewise linear function with $O(n)$ inflection points (on the nonnegative half line) that can be constructed in $O(n^2)$ time. Its  maximum value in 
$\left[ w_i^-,\,w_i^+\right]$ can therefore be calculated in $O(n)$ further time, proving (1).

The proof of (2) is symmetric.
\end{proof}

\begin{lemma}
\label{lem:Gij}
Fix $x$  Let $x_i < x_j \le x$.  The 
\begin{enumerate}
\item   $G_{i,j}(x)$ can be calculated in $O(n^2)$ time.
\item  $H_{i,j}(x)$ can be calculated in $O(n^2)$ time.
\end{enumerate}
\end{lemma}
\begin{proof}
Set $s = s_{i,j}(0,w_j^+).$ Recall that
\begin{eqnarray*}
G_{i,j} (x) &=& \max_{ s \in S_{i,j}, w_j(s) = w_j^+} \left\{ g_j(x:s) - \min_{y \ge x_j} \Theta(P,y:s) \right\}\\
&=&  \max_{\alpha \in \left[ w_i^-,\,w_i^+\right]} \left\{ g_j(x:s_{-i}(\alpha)) - \min_{y \ge x_j} \Theta(P,y:s_{-i}(\alpha))  \right\}.
\end{eqnarray*}
The proof that  $G_{i,j}(x)$  and similarly  $H_{i,j}(x)$ can be calculated in $O(n^2)$ time is then the same as the proof of  \Cref {lem:Gj}.
\end{proof}

This immediately yields
\begin{corollary}
\label{cor:GH}
For any fixed $x$,  $G(x)$ and $H(x)$ can be calculated in $O(n^4)$ time.
\end{corollary}

\subsection{Efficient Computation of $\bar G(x)$ and $\bar H(x)$}
Recall that, for fixed $x$ and  $i < j$ with $x_j \le x$
$$\bar G_{i,j}(x) = \max_{ s \in S_{i,j}} \left\{ \left(\max_{t\,:\, x_j \le x_t \le x} g_t(x:s)\right) - \min_{y: x_i \le y \le x_j} \Theta(P,y:s) \right\}$$


It is straightforward to prove
\begin{lemma}
\label{lem:combine}
 Let $x, i, j,t$ be fixed and satisfy  $i < j \le t$ with $x_t \le x$. Also set $t' = \max\{j \,: x_{j'} < x\}.$
  Then
 \begin{eqnarray*}
g_t \left(x: s_{i,j}(\alpha_1,  \alpha_2)\right) &=& d(x_t,x) +  a_t W_{0,t}(s)  +  a_t \left( \alpha_1 + \alpha_2) - (w^-_i+w^-_j)  \right)\\
 &=& \left(  d(x_t,x) +  a_t \Bigl(W_{0,t}(s)   -  (w^-_i+w^-_j)\Bigr)  \right) + a_t  \Bigl( \alpha_1 + \alpha_2 \bigr).
 \end{eqnarray*}
 where $a_j = \frac 1  {\tilde c_{t,t'}}$.
 Thus
$$\max_{t\,:\, x_j \le x_t \le x} g_t \left(x: s_{i,j}(\alpha_1,  \alpha_2\right) = F(\alpha_1 + \alpha_2)$$
where $F(\beta)$ is the upper-envelope of $O(t'-j)=O(n)$ lines that can be constructed in $O(n)$ time.
\end{lemma}




\begin{lemma}
\label{lem:barGij}
Let $x, i, j$ be fixed and satisfy  $i < j$ with $x_j \le x$. Suppose $y\in I = [x_i,x_j]$ and $s\in S_{i,j}$ satisfy the restrictions in the definition of $\bar G_{i,j}(x)$ and achieve the maximum value, i.e., 
$$  \left(\max_{t\,:\, x_j \le x_t \le x} g_t(x:s)\right)  - \Theta(P,y:s)  = \bar G_{i,j}(x).$$
Then $s = s_{i,j}(\alpha_1,\alpha_2)$ where $\alpha_1 \in \left[ w_i^-,\,w_i^+\right]$,  $\alpha_2 \in \left[ w_j^-,\,w_j^+\right]$ and at least one of the following three conditions is true:
\begin{enumerate}
\item[(C1)]  $\alpha_1 = w_i^+,$
\item[(C2)]  $\alpha_2 = w_j^+,$ or
\item[(C3)]  $\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) = \Theta_R\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right).$
\end{enumerate}
\end{lemma}
\begin{proof}
All $s \in S_{i,j}$ are in the form $s = s_{i,j}(\alpha_1,\alpha_2)$ where $\alpha_1 \in \left[ w_i^-,\,w_i^+\right]$,  $\alpha_2 \in \left[ w_j^-,\,w_j^+\right]$.
Thus, to prove the lemma, it suffices to prove that, for all $y \in I,$  and  $\alpha_1,\alpha_2$,  the maximum of  
$$F(\alpha_1 + \alpha_2) - \Theta \left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right)$$
is only achieved when at least one of conditions (C1), C(2), (C3) holds.


Recall that 
$$\Theta \left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) = \max\left( \Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right),\, \Theta_R\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right)\right).
$$
Because $x_i \le y \le x_j,$
\begin{itemize}
\item  $\forall \alpha_2 \ge  0,\,  \Theta_L \left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) =\Theta_L \left(P,y:s_{i,j}(\alpha_1,0)\right), $
\item  $\forall \alpha_1 \ge  0,\,  \Theta_R \left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) =\Theta_R \left(P,y:s_{i,j}(0,\alpha_2)\right),$
\end{itemize}
 Furthermore, for fixed $y,$
 $\Theta_L \left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right)$  (resp.  $\Theta_R \left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right)$)  is a continuous, piecewise linear, monotonically increasing function of $\alpha_1$ (resp.  $\alpha_2$).


Suppose that the left and right evacuation times are not equal  and, without loss of generality,
$$\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) >\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right).$$
Continuously increase $\alpha_2$  to $\bar \alpha_2$ until either
$$\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) =\Theta_L\left(P,y:s_{i,j}(\alpha_1, \bar \alpha_2)\right)$$
or  $\bar \alpha_2 = w^+_j$.
Note that,  
$$\Theta \left(P,y:s_{i,j}(\alpha_1, \bar \alpha_2)\right) = \Theta \left(P,y:s_{i,j}(\alpha_1,  \alpha_2)\right).$$
From \Cref{lem:combine}, if $\bar \alpha_2 > \alpha_2$ then  $F(\alpha_1 + \bar \alpha_2) > F(\alpha_1 + \alpha_2).$
%The crucial observation is that, for every $t$ satisfying $x_j \le x_t$ ,   $g_t\left(x: s_{i,j}(\alpha_1,  \alpha_2\right)$ is a linear function (with positive slope) of $\alpha_1 + \alpha_2$.
%Thus
%$$\max_{t\,:\, x_j \le x_t \le x} g_t \left(x: s_{i,j}(\alpha_1,  \bar \alpha_2\right) \ge \max_{t\,:\, x_j \le x_t \le x} g_t \left(x: s_{i,j}(\alpha_1,  \alpha_2\right)$$
%with equality possible only if  (C2) or (C3) holds.  
Thus
$$ F(\alpha_1 +\bar  \alpha_2) -\Theta \left(P,y:s_{i,j}(\alpha_1, \bar  \alpha_2)\right)
\ge 
F(\alpha_1 + \alpha_2) -\Theta \left(P,y:s_{i,j}(\alpha_1,  \alpha_2)\right)$$
with equality possible only if, $\alpha_2 = \bar \alpha_2,$ i.e.,  (C2) or (C3) holds.   
Equality not holding would contradict the choice of $s$ and $y$ and therefore either (C2) or (C3)   must hold.



A symmetric argument when 
$$\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) <\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right)$$
permits increasing $\alpha_1$ to $\bar \alpha_1$ 
until either
$$\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) =\Theta_L\left(P,y:s_{i,j}(\bar \alpha_1, \alpha_2)\right)$$
or  $\bar \alpha_1 = w^+_i$ which would then prove that  either (C1) or (C3)   must hold.

Thus one of  (C1), (C2) or (C3)   must hold.
\end{proof}



\begin{lemma}
\label{lem:bar construction}
Let $x, i, j$ be fixed and satisfy  $i < j$ with $x_j \le x$. Then $\bar G_{i,j}(x)$ and $\bar H_{i,j}(x)$ can each be calculated in $O(n^2)$ time.
\end{lemma}
\begin{proof}
We only show how to evaluate $\bar G_{i,j}(x)$. The evaluation of  $\bar H_{i,j}(x)$ is totally symmetric.

In what follows we always set $s=s_{i,j}\left(0,0\right)$ and
%Before starting,  let $s=s_{i,j}\left(w^-_i,w^-_j\right)$ and 
for all $t,$  $i \le t \le j$ define
\begin{eqnarray*}
\lue_{i,t}(\alpha) &=&  \Theta_L(P,x_t :s_{-i} (\alpha)), \\
\rue_{j,t}(\alpha) &=&  \Theta_R(P,x_t :s_{-j} (\alpha)).
\end{eqnarray*}
Note that, for all $\alpha_1,\alpha_2 \ge 0$ this implies
\begin{eqnarray*}
\lue_{i,t}(\alpha_1) &=&  \Theta_L(P,x_t :s_{i,j} (\alpha_1,\alpha_2))\\
\rue_{j,t}(\alpha_2) &=&    \Theta_R(P,x_t :s_{i,j} (\alpha_1,\alpha_2)).
\end{eqnarray*}
From \Cref{obs:LUE} these are both upper envelopes of $O(n)$  lines with non-negative slopes.  Furthermore, 
%from \Cref{lem:UE} and the discussion following it, these can all be built in $O(n^2)$ total time.
for each fixed $t$ they can be built in $O(n)$ time so all of them can be built in $O(n^2)$ total time.

We need to construct
\begin{eqnarray*}
\bar G_{i,j}(x) &=& 
 \max_{ s \in S_{i,j}} \left\{ \left(\max_{t\,:\, x_j \le x_t \le x} g_t(x:s)\right) - \min_{y: x_i \le y \le x_j} \Theta(P,y:s) \right\},\\
 &=&
\max_{ \substack{ { \alpha_1\in  \left[ w^-_i,w^+_i\right]}   \\  { \alpha_2\in  \left[ w^-_j,w^+_j\right]}}}
% \max_{ \alpha_1\in  \left[ w^-_i,w^+_i\right],\, \alpha_2\in  \left[ w^-_j,w^+_j\right]} 
 \left\{ 
F(\alpha_1 + \alpha_2)  - \min_{y \in I} \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2))
  \right\}
\end{eqnarray*}
where $I=[x_i,x_j].$

From \Cref{lem:combine}  $F(\beta)$ is  a piecewise linear function with $O(n)$ inflection points that can be constructed in  $O(n)$ time.


From \Cref{lem:barGij} we can restrict ourselves to calculating the maximum value in the three cases
(i) $\alpha_1 = w_i^+,$ (ii)
 $\alpha_2 = w_j^+,$ or
(iii) $\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) = \Theta_R\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right).$

\medskip


\par\noindent\underline{Step 1:} $\alpha_1 = w_i^+:$\\
We need to calculate
$$ \max_{\alpha_2\in  \left[ w^-_j,w^+_j\right]} \left( F(w^+_i +\alpha_2)-
\min_{y \in I} \Theta(P,y:s_{i,j}(w^+_i,\alpha_2))\right). $$

$F(w^+_i +\alpha_2)$ is  piecewise linear function with $O(n)$ inflection points that can be constructed in $O(n )$ time from $F(\beta).$  

From  \Cref{lem:yalpha5} , after appropriate relabelling,  
$\min_{y \in I} \Theta(P,y:s_{i,j}(w^+_i,\alpha_2)) = \Theta(\alpha_2)$
 where $\Theta(\alpha_2)$ is  piecewise linear function with $O(n)$ inflection points that can be constructed in $O(n^2)$ time.

After constructing these two functions we can then, in $O(n)$ time, construct the function
\begin{equation}
\label{eq:FThetadiff}
F(w^+_i +\alpha_2)-
\min_{y \in I} \Theta(P,y:s_{i,j}(w^+_i,\alpha_2)
\end{equation}
which is also a piecewise linear function with $O(n)$ inflection points.  After constructing it, we can find the value $ \alpha_2\in  \left[ w^-_j,w^+_j\right]$ at which it achieves its maximum in $O(n)$ further time.

{\em Note: it might seem possible that the maximum could be found in $o( \log n)$ time.  Unfortunately, the function defined in \Cref{eq:FThetadiff}  is the difference between two piecewise linear monotonically increasing functions, could possess many local maxima, and does not seem to possess a special structure.}


\medskip


\par\noindent\underline{Step 2:} $\alpha_2 = w_j^+:$\\
We need to calculate
$$ \max_{\alpha_1\in  \left[ w^-_i,w^+_i\right]} 
\left( 
F(\alpha_1 + w^+_j)-
\min_{y \in I} \Theta(P,y:s_{i,j}(\alpha_1,w^+_j))
\right). 
$$
Finding the value $ \alpha_1\in  \left[ w^-_i,w^+_i\right]$ at which it achieves its maximum can be done in in $O(n^2)$ time exactly as $\alpha_2$ was found in Step 1.

\medskip


\par\noindent\underline{Step 3:} $\alpha_1 = w_i^-$ or  $\alpha_2 = w_j^i:$\\
For the next case we will also need to have checked 
$$ \max_{\alpha_1\in  \left[ w^-_i,w^+_i\right]} 
\left( 
F(\alpha_1 + w^-_1)-
\min_{y \in I} \Theta(P,y:s_{i,j}(\alpha_1,w^-_j))
\right)
$$
and
$$ \max_{\alpha_1\in  \left[ w^-_i,w^-_i\right]} 
\left( 
F(\alpha_1 + w^+_j)-
\min_{y \in I} \Theta(P,y:s_{i,j}(\alpha_1,w^-_j))
\right). 
$$
These can be checked in a further $O(n^2)$ time exactly as in steps 1 and 2.
\medskip

\par\noindent\underline{Step 4:}  $\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) = \Theta_R\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right).$


We observe that if $\alpha_1,\alpha_2$ are fixed then it is possible that no $y$  satisfying 
\begin{equation}
\label{eq:LREQX} \Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) = \Theta_R\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right)
\end{equation}
exists.
If such a $y$ does exist it is unique and we denote it by $y(\alpha_1,\alpha_2).$

Our goal is to calculate
\begin{equation}
\label{eq:FG2cc}
X= \max_{ \substack{ { \alpha_1\in  \left[ w^-_i,w^+_i\right]},    { \alpha_2\in  \left[ w^-_j,w^+_j\right] }\\y(\alpha_1,\alpha_2)  \in I }}
% \max_{ \alpha_1\in  \left[ w^-_i,w^+_i\right],\, \alpha_2\in  \left[ w^-_j,w^+_j\right]} 
 \left\{ 
F(\alpha_1 + \alpha_2)  %- \min_{y \in I} \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2))
-\Theta(P,y(\alpha_1,\alpha_2) :s_{i,j}(\alpha_1,\alpha_2))
  \right\}.
\end{equation}
in $O(n^2)$ time.  Combined with the results of Steps 1 and 2 this will cover all three cases (i) (ii) and (iii) and thus complete the proof of the Lemma


\medskip
In what follows we will show how, for  every  $t$ satisfying $i \le t \le j$,  to calculate  
\begin{equation}
\label{eq:FG2ccc}
A_t =\max_{ \substack{ { \alpha_1\in  \left[ w^-_i,w^+_i\right]},    { \alpha_2\in  \left[ w^-_j,w^+_j\right] }\\y(\alpha_1,\alpha_2)  =x_t  }}
% \max_{ \alpha_1\in  \left[ w^-_i,w^+_i\right],\, \alpha_2\in  \left[ w^-_j,w^+_j\right]} 
 \left\{ 
F(\alpha_1 + \alpha_2)  %- \min_{y \in I} \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2))
-\Theta(P,y(\alpha_1,\alpha_2) :s_{i,j}(\alpha_1,\alpha_2))
  \right\}.
\end{equation}
in $O(n)$ time and also,   every  $t$ satisfying $i \le t < j$ 
to calculate  the contribution to $ \bar G_{i,j}(x)$ from 
\begin{equation}
\label{eq:FG2cccc}
B_t = \limsup_{ \substack{ { \alpha_1\in  \left[ w^-_i,w^+_i\right]},    { \alpha_2\in  \left[ w^-_j,w^+_j\right] }\\y(\alpha_1,\alpha_2)  \in  I_t  }}
% \max_{ \alpha_1\in  \left[ w^-_i,w^+_i\right],\, \alpha_2\in  \left[ w^-_j,w^+_j\right]} 
 \left\{ 
F(\alpha_1 + \alpha_2)  %- \min_{y \in I} \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2))
-\Theta(P,y(\alpha_1,\alpha_2) :s_{i,j}(\alpha_1,\alpha_2))
  \right\}.
\end{equation}
in $O(n)$ time. 
The reason for writing $\limsup$ instead of $\max$ in  \Cref{eq:FG2cccc} is that 
technically, because $I_t$ is an {\em open} interval, and all of the functions involved are continuous, it is possible 
that  `` $\max$''  does not exist because the set of values being maximized over, while bounded, is open.

We will, though, show that if $B_t > \max\{A_t,A_{t+1}\}$ then 
$$B_t = F(\alpha_1 + \alpha_2)  
-\Theta(P,y(\alpha_1,\alpha_2) :s_{i,j}(\alpha_1,\alpha_2))$$
for some $(\alpha_1,\alpha_2)$ and $y \in I_t$ and thus 
\begin{equation}
\label{eq:FGh}
X =\max \left(    \max_{1 \le t \le j} A_t,\, \max_{i \le t < j } B_t\right).
\end{equation}
This will then permit calculating $X$ in $O(n^2)$ time, completing the proof  of the Lemma.




%For  all that follows set $s= s_{i,j}(0,0)$.
\medskip

\underline{(a)  Evaluating $A_t$:}
Fix $t$ satisfying $i \le t \le j.$  %Assume $y(\alpha_1,\alpha_2)=x_t$    
%Set $s= s_{i,j}(\alpha_1,\alpha_2)$.

Evaluating $A_t$ will require being able to calculate the value of $\alpha_1+ \alpha_2$ when
$$  \Theta_L\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right) =  \Theta_R\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right).$$

 

\medskip


Note that $\forall \alpha_1 \ge 0,\, \alpha_2 \ge 0,$
\begin{eqnarray*}
\Theta_L\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right) &=&  \lue_{i,t}(\alpha_1),\\
\Theta_R\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right) &=&  \rue_{i,t}(\alpha_1).
\end{eqnarray*}


Recall that $ \lue_{i,t}(\alpha)$ and $\rue_{i,t}(\alpha)$ have already been built and each of these functions is a monotonically increasing linear function in $\alpha$ with $O(n)$ inflection points.
Set  $\beta_L = \lue_{i,t}(0)$  and $\beta_R = \rue_{i,t}(0).$




% $ \lue_{i,t}(\alpha_1) = \tau$ only has a has a solution $\alpha_1 \ge 0$ if $\tau \ge \beta_L$ and,if the solution e, the solution is unique.
%
%
%
%Consider time $\tau_L  \ge 0$.  If there exists an $\alpha_1$ such that $\Theta_L\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right)= \tau_L$ then $\alpha_1$ is unique and $\alpha_1$ increases with $\tau_L.$ 
%Similarly,  for any $\tau_R  \ge 0$, if there exists an $\alpha_2$ such that $\Theta_L\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right)= \tau_R \ge 0$ then $\alpha_2$ is unique and $\alpha_2$ increases with $\tau_R.$
%So, for any $\tau \ge 0,$ requiring  $\tau_L =\tau_R=\tau$ fixes  a unique amount of flow that can reach $x_t$ in time $\tau$ (if evacuation in time $\tau$ is possible).
%This will enable us  to quickly evaluate $A_t$.  The details are developed below.
%

% Furthermore
%\begin{eqnarray*}
%\lue_{i,t}(\alpha_1) &=& \Theta_L\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right)\\
%\rue_{i,t}(\alpha_2) &=& \Theta_R\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right).
%\end{eqnarray*}

\medskip

From the properties of $\lue_{i,t}(\alpha_1)$, 
\begin{itemize}
\item  $T_L(\tau)$, the inverse of  $\lue_{i,t}(\alpha_1)$,  satisfying $\lue_{i,t}(T_L(\tau)) =z$, exists in the range
$z \in [\beta_L, \infty]$. % where $\beta_L = \lue_{i,t}(0).$
\item $T_L(\tau)$ is a piecewise linear monotonically increasing function with  $O(n)$ inflection points
\item  $T_L(\tau)$ can be built in $O(n)$ time from $\lue_{i,t}(\alpha_1)$,
\end{itemize}
Similarly,
\begin{itemize}
\item  $T_R(\tau)$, the inverse of  $\rue_{i,t}(\alpha_2)$,  satisfying $\rue_{i,t}(T_R(\tau)) =z$, exists in the range
$z \in [\beta_R, \infty]$. % where $\beta_R = \rue_{i,t}(0).$
\item $T_R(\tau)$ is a piecewise linear monotonically increasing function with  $O(n)$ inflection points
\item  $T_R(\tau)$ can be built in $O(n)$ time from $\rue_{i,t}(\alpha_1)$,
\end{itemize}

%Let $\tau \ge 0.$  
%$T_L(\tau)$ is the unique solution $\alpha_1$ to  $\lue_{i,t}(\alpha_1) = \tau$. 
%$T_R(\tau)$ is the unique solution $\alpha_2$ to  $\rue_{i,t}(\alpha_2) = \tau$.

 Set $T(\tau) = T_L(\tau) + T_R(\tau)$.  $T(\tau)$  is defined in the range
$\tau  \in [\beta, \infty]$ where $\beta = \max(\beta_L,\beta_R)$.


 %and is the amount of flow evacuating to $x_t$ in time $\tau$ when  $\lue_{i,t}(\alpha_1) = \tau = \rue_{i,t}(\alpha_2) $.


 Since $T(z)$ is the sum of two monotonically increasing piecewise linear functions, each with $O(n)$ inflection points, $T(z)$ is also a monotonically increasing piecewise linear function with $O(n)$ inflection points.  It can be built from $T_L(z)$ and $T_R(z)$ via an $O(n)$ time merging procedure.

\medskip


By construction   $\lue_{i,t}(\alpha_1) = \tau = \rue_{i,t}(\alpha_2) $ only has a solution if  $\tau  \in [\beta, \infty]$ and, for each such such $\tau$, $\alpha_1,\beta_1$ are unique and 
$$\alpha_1 + \alpha_2 = T_L(\tau) + T_R(\tau) = T(\tau).$$
Since $T(\tau)$ is monotonically increasing this implies that  there can be at most one solution $G(\alpha)$ to
$$G(\alpha) = \alpha_1 + \alpha_2
\quad \mbox{where}   \quad 
\lue_{i,t}(\alpha_1) = \rue_{i,t}(\alpha_2)  \ \ \mbox{and}\ \  
\alpha_1 + \alpha_2 = \alpha.$$


 $G(\alpha)$ is the inverse of $T(\tau)$.
This is defined in the range  $\alpha \ge T(\beta)$, is also a monotonically increasing piecewise linear function with $O(n)$ inflection points  and can be built from $T(z)$ in $O(n)$ time.
%  By construction $G(\alpha)$ is the {\em unique} amount of time required for evacuating $s_{i,j}(\alpha_1,\alpha_2)$ to $x_t$  when $\alpha= \alpha_1 + \alpha_2$ and 
% $$\Theta_L\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right) = \Theta_R\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right).$$


% $\Theta_L\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right) = \Theta_R\left(P,x_t:s_{i,j}(\alpha_1,\alpha_2)\right) = \tau \ge 0,$ then 
%$\alpha_1 + \alpha_2 = T(\tau)  \ge T(\beta).$ 
Now set $\kappa_L, \kappa_R, \kappa, \gamma_L, \gamma_R, \gamma$ to be the unique values such that

\begin{align*}
T_L(\kappa_L) &= w^-_i, &	 T_R(\kappa_R) &= w^-_j,	& \kappa &=\max\left( \kappa_L, \kappa_R\right),\\
T_L(\gamma_L) &= w^+_i, &	 T_R(\gamma_R) &= w^+_j,	& \gamma &=\min\left( \gamma_L, \gamma_R\right).
\end{align*}




% Further set,
%$\gamma_L$ to be the unique value such that $T_L(\gamma_L) = w^+_i$ and $\gamma_R$ to be the unique value such that $T_R(\gamma_R) = w^+_j$ and $\gamma = \min\left( \gamma_L, \gamma_R\right).$

\medskip


\medskip

%$\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) = \LUE_{i,m}(\alpha_1).$
Thus,  fixing $x_t$ and restricting
we find
\begin{equation}
\label{eq:FGa}
%\max_{ \alpha_1\in  \left[ w^-_i,w^+_i\right],\, \alpha_2\in  \left[ w^-_j,w^+_j\right]} 
A_t =
\max_{ \substack{ { \alpha_1\in  \left[ w^-_i,w^+_i\right]},    { \alpha_2\in  \left[ w^-_j,w^+_j\right] }\\y(\alpha_1,\alpha_2)  =x_t  }}
 %\max_{ \substack{ { \alpha_1\in  \left[ w^-_i,w^+_i\right]}   \\  { \alpha_2\in  \left[ w^-_j,w^+_j\right]}}}
 \left\{ 
F(\alpha_1 + \alpha_2)  -  \Theta(P,x_t:s_{i,j}(\alpha_1,\alpha_2))
  \right\}
  =
  \max_{\kappa \le \alpha \le \gamma} \left(F(\alpha) - G(\alpha)\right).
 \end{equation}
  Since both $F(\alpha)$ and $G(\alpha)$ are known piecewise linear functions with $O(n)$ inflection points, the maximum value can be found in $O(n)$ time.
  
  Note that it is possible that $\gamma < \kappa.$ In this case no scenario satisfying the constraints exists.
  

\bigskip


\underline{(b)  Evaluating $B_t$: }  Fix $t$ satisfying $i \le t < j.$  
%Let  $I = \left(x_t, x_{t+1}\right)$  and  $\bar I = [x_t,x_{t+1}].$ Set  $s= s_{i,j}(0,0)$. 

%  In what follows we want to calculate the contribution to $ \bar G_{i,j}(x)$ from 
%\begin{equation}
%\label{eq:FG2}
%\max_{ \substack{ { \alpha_1\in  \left[ w^-_i,w^+_i\right]},    { \alpha_2\in  \left[ w^-_j,w^+_j\right]} \\ y(\alpha_1,\alpha_2) \in I}}
%% \max_{ \alpha_1\in  \left[ w^-_i,w^+_i\right],\, \alpha_2\in  \left[ w^-_j,w^+_j\right]} 
% \left\{ 
%F(\alpha_1 + \alpha_2)  %- \min_{y \in I} \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2))
%- \Theta(P,y(\alpha_1,\alpha_2) :s_{i,j}(\alpha_1,\alpha_2))
%  \right\}.
%\end{equation}

%We may restrict ourselves to maximal cases that were not already found in  Steps 1,2,3 and 4(a).
%*********We thus  may assume that   $\alpha_1 \not= w^+_i,w^-_i$ and $\alpha_2\not= w^+_j,w^-_j$.**********

Note that 
technically, because $I_t$ is an {\em open} interval, and all of the functions involved are continuous, it is possible 
that the `` $\max$''  in \Cref{eq:FG2cccc} does not exist because the set of values being maximized over, while bounded, is open.
 We deal with this issue shortly by extending the interval from the open $I_t$ to the closed $\bar I_t$  and then show that if the $\max$ exists at the endpoints $x_t,x_{t+1}$ of  $\bar I_t$ then the max will be dominated by  one of the values found in part (a) above and therefore can be ignored.



%
%
%We therefore augment the function to be defined over all of $\bar I$ by defining 
%
%$$\bar \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2)) =
%\left\{
%\begin{array}{ll}
% \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2))    & \mbox{ if $ \in I$}\\
%\lim_{y \downarrow x_t}  \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2))  & \mbox{ if $y =x_t$}\\
%\lim_{y  \uparrow x_t}  \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2))  & \mbox{ if $y =x_{t+1}$}
%\end{array}
%\right.,
%$$
%and replacing 
%\Cref{eq:FG2a}  with
%\begin{equation}
%\label{eq:FG2}
%\max_{ \substack{ { \alpha_1\in  \left[ w^-_i,w^+_i\right]}   \\  { \alpha_2\in  \left[ w^-_j,w^+_j\right]}}}
%% \max_{ \alpha_1\in  \left[ w^-_i,w^+_i\right],\, \alpha_2\in  \left[ w^-_j,w^+_j\right]} 
% \left\{ 
%F(\alpha_1 + \alpha_2)  - \min_{y \in \bar I}   \bar \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2))
%  \right\}.
%\end{equation}



From \Cref{cor:smooth evac}, for $y \in I_t,$ 
\begin{eqnarray*}
\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) &= &  \Theta_L\left(P,x_{t+1}:s_{i,j}(\alpha_1,\alpha_2)\right) - (x_{t+1}-y),\\
\Theta_R\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) &=&   \Theta_R\left(P,x_{t}:s_{i,j}(\alpha_1,\alpha_2)\right)  - (y- x_t).
\end{eqnarray*}
Recall too that, for $y \in I_t,$ 
 $$\Theta_L\left(P,x_{t+1}:s_{i,j}(\alpha_1,\alpha_2)\right) = \lue_{i,t+1}(\alpha),\quad 
\Theta_R\left(P,x_{t}:s_{i,j}(\alpha_1,\alpha_2)\right) = \rue_{i,t}(\alpha).$$
Set
$$%\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right)  = 
f_L(\alpha)  =  \lue_{i,t+1}(\alpha) - x_{t+1},\quad
%\Theta_R\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right)  = 
f_R(\alpha) =  \rue_{i,t+1}(\alpha) + x_{t}.
$$
%and the continuity of  $f_L,$  $f_R$ 
This  permits writing
\begin{eqnarray*}
\Theta_L\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) &= &  f_L(\alpha_1) + y,\\
\Theta_R\left(P,y:s_{i,j}(\alpha_1,\alpha_2)\right) &=&    f_R(\alpha_2) - y.
\end{eqnarray*}
$\lue_{i,t+1}(\alpha)$  and $\rue_{i,t}(\alpha)$ have already been built and are monotonically increasing piecewise linear functions with $O(n)$ inflection points.
$f_L(\alpha)$ and $f_R(\alpha)$ are therefore also monotonically increasing piecewise linear functions with  the same slopes and $O(n)$ inflection points.

\Cref {eq:LREQX} becomes 
\begin{equation}
\label{eq:Case 2eq}
f_L(\alpha_1) + y  = f_R(\alpha_2) - y.
\end{equation} 
so $y(\alpha_1,\alpha_2)$ when it exists,  solves to $y(\alpha_1,\alpha_2) = \bar y(\alpha_1,\alpha_2)$ where 
\begin{equation}
\label{eq:yalph}
\bar y(\alpha_1,\alpha_2) =  \frac 1 2 ( f_R(\alpha_2)  -  f_L(\alpha_1)).
\end{equation}
Thus
$$ \Theta(P,y(\alpha_1,\alpha_2) :s_{i,j}(\alpha_1,\alpha_2))
= f_L(\alpha_1) + y(\alpha_1,\alpha_2)  = \frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1))
$$

%Substitute this into 
%  \Cref{eq:FG2cccc}  to 
  
  Now define 
\begin{equation}
\label{eq:FG2b}
B'_t = \max_{ \substack{ { \alpha_1\in  \left[ w^-_i,w^+_i\right]},\,   { \alpha_2\in  \left[ w^-_j,w^+_j\right]} \\ y(\alpha_1,\alpha_2) \in \bar I_t}}
% \max_{ \alpha_1\in  \left[ w^-_i,w^+_i\right],\, \alpha_2\in  \left[ w^-_j,w^+_j\right]} 
 \left\{ 
F(\alpha_1 + \alpha_2)  %- \min_{y \in I} \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2))
%\Theta(P, \bar y(\alpha_1,\alpha_2) :s_{i,j}(\alpha_1,\alpha_2))
 - \left(\frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1))\right)
  \right\}.
\end{equation}
Note the replacement of $ y(\alpha_1,\alpha_2) \in I_t$  by $  y(\alpha_1,\alpha_2) \in \bar I_t$.
Taking the maximum over  a closed interval guarantees that   $B'_t$ exists.  Furthermore, since all of the functions involved are continuous, $B'_t = B_t.$

%
%  If $y(\alpha_1,\alpha_2) \in I$
%then  $ \bar y(\alpha_1,\alpha_2) = y(\alpha_1,\alpha_2)  \in I$.
%If  $y(\alpha_1,\alpha_2) \not \in  I$ but $ \bar y(\alpha_1,\alpha_2)  \in \bar I$ then $ \bar y(\alpha_1,\alpha_2) \in \{x_t,x_{t+1}\}.$
%Thus, if` $B'_t \not = B_t$ then  $B'_t > B_t$  and the maximum in  \Cref{eq:FG2cccc}  must be achieved at either  $x_t$ or $x_{t+1}.$

We claim that if the maximum is achieved for some $\alpha_1,\alpha_2$ pair with $\bar y(\alpha_1,\alpha_2) = x_t$ then $ B'_t \le A_t.$   This is because, by  definition and continuity, for all $\alpha_1,\alpha_2$,
$$  \Theta(P,x_t:s_{i,j}(\alpha_1,\alpha_2))
 \le  \lim_{ \substack{  y \downarrow x_t \\  \alpha_1' \rightarrow \alpha_1  \\ \alpha_2' \rightarrow \alpha_2}}   \Theta(P,y:s_{i,j}(\alpha_1,\alpha_2))$$
where it doesn't matter in what order the limits are taken. Similarly, 
 if the maximum is achieved for some $\alpha_1,\alpha_2$ pair with $\bar y(\alpha_1,\alpha_2) = x_{t+1}$ then  $B'_t \le A_{t+1}$.
 
Thus, if $B_t > \max\{A_t,A_{t+1}\}$ then 
$$B'_t = B_t = F(\alpha_1 + \alpha_2)  
-\Theta(P,y(\alpha_1,\alpha_2) :s_{i,j}(\alpha_1,\alpha_2))$$
for some $(\alpha_1,\alpha_2)$ and $y \in I_t$, which is what was required.

%
%We can therefore replace  $B_t$ by $B'_t$ in  \Cref{eq:FGh}    to find
%\begin{equation}
%X =\max \left(    \max_{1 \le t \le j} A_t,\, \max_{i \le t < j } B'_t\right) 
%\end{equation}
%Since we are only interested in calculating $X$ and not $B_t$ we may restrict ourselves in this section to calculating $B'_t.$

The major issue in evaluating \Cref{eq:FG2b} in $O(n)$ time is that there does not seem to be any relationship between $\alpha_1$ and $\alpha_2$. 
 In the sequel, we how that, for any given $\alpha$  there only exist $O(1)$ possible pairs $(\alpha_1,\alpha_2)$ within the specified range such that $\alpha_1 + \alpha_2 = \alpha$ and the pair could contribute to the maximum.



 %If such a $y \in \bar I$ exists we  denote it by $y(\alpha_1,\alpha_2)$ and say that $\alpha_1,\alpha_2$ is a {\em legal pair}.






\begin{definition}
\ 
\begin{itemize}
  \item $\alpha_1,\alpha_2$  is a {\em legal  pair} if  $y(\alpha_1,\alpha_2) \in \bar I_t$

 \item $\alpha_1,\alpha_2$  is a {\em good   pair} if it is  a legal pair and $ \forall \alpha'_1,\alpha'_2$ such that   $y(\alpha'_1,\alpha_2') \in \bar I_t$ and $\alpha'_1 + \alpha'_2 = \alpha_1 + \alpha_2$
$$  f_R(\alpha_2)  +  f_L(\alpha_1) \le  f_R(\alpha'_2)  +  f_L(\alpha'_1).$$

\item For   $\alpha$ satisfying  $w^-_i + w^-_j \le  \alpha \le w^+_i + w^+_j$ set
$$
G(\alpha) =
\left\{
\begin{array}{ll}
\mbox{undefined} & \mbox{If no legal  pair $\alpha_1,\alpha_2$ with $\alpha_1 + \alpha_2 = \alpha$ exists}\\
\frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1)) &\mbox{If good pair $\alpha_1,\alpha_2$ with $\alpha_1 + \alpha_2 = \alpha$ exists}
\end{array}
\right.
$$

\end{itemize}
\end{definition}
By the continuity of the functions we note that if, for some $\alpha$  a legal pair $\alpha_1,\alpha_2$ satisfying $\alpha_1 + \alpha_2 = \alpha$ exists then a good pair $\alpha'_1,\alpha'_2$ satisfying $\alpha'_1 + \alpha'_2 = \alpha$ also exists so $G(\alpha)$ is well defined.
Working through the definitions we can now 
replace  \Cref{eq:FG2b}  by
\begin{equation}
\label{eq:FG2replace}
B'_t = \max_{ w^-_i + w^-_j \le  \alpha \le w^+_i + w^+_j} (F(\alpha) - G(\alpha))
\end{equation}
It thus remains to quickly evaluate $G(\alpha).$



Before starting we divide  legal pairs into 7 different types of cases. These are
%
%We have therefore just seen that if $G(\alpha)$ is defined then 
%$G(\alpha) = 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1))$   where at least one of the following  four conditions apply
\begin{itemize}
\item [(1)] $\alpha_1 = w^-_i$ 
\item [(2)]   $\alpha_1 = w^+_i$ 
\item [(3)]  $\alpha_2 = w^-_j$ 
\item [(4)]  $\alpha_1 = w^+_j$ 
\item [(5)]  $y(\alpha_1,\alpha_2) =  \frac 1 2 ( f_R(\alpha_2)  -  f_L(\alpha_1)) = x_t$
\item [(6)]  $y(\alpha_1,\alpha_2) =  \frac 1 2 ( f_R(\alpha_2)  -  f_L(\alpha_1)) = x_{t+1}$
\item [(7)]  All legal pairs that are not in Cases 1-6.
\end{itemize}
For each case  $i\in \{1,2,3,4,5,6\}$  we note that, for each $\alpha$, at most one legal pair $\alpha_1,\, \alpha - \alpha_1$ exists.  This is obviously true for cases 1-4.  For cases $5,6$ it follows from the fact that $ f_L(\alpha_1)$  and $ f_R(\alpha_2)$ are both monotonically increasing continuous functions. Let $(\alpha_i^{(i)},\alpha_2^{(i)})$ denote the unique  case $i$ legal pair such that $\alpha_i^{(i)} + \alpha_2^{(i)} = \alpha$ if such exists.   Then $\alpha_i^{(i)}$ and $\alpha_2^{(i)}$ are piecewise linear functions with $O(n)$ inflection points that can be built in $O(n)$ time from knowledge of
 $ f_L(\alpha_1))$ and $ f_R(\alpha_2)$ (in cases $1,2,3,4$ they are even simpler).
Also  the range of $\alpha$  for which each case $i$ holds is a closed interval ${\mathcal I}^{(i)}.$   %For case $i\in \{1,2,3,4,5,6\}$   and $\alpha\in {\mathcal I}^{(i)}$
 


%{\color{red}  This is not hard to prove but tedious for Cases 5,6.}
%
%
%To see this for case 1 note that
% $\alpha_1 = w^-_i$, implies $\alpha_2 = \alpha - w^-_i$ so 
%$$ x_t \le \bar y(w^-_i,\alpha_2)  \le x_{t+1} 
%\quad \Leftrightarrow \quad
%2 \left(x_t + f_L\left(w^-_i\right)\right)  \le f_R(\alpha- w^-_i) \le 2 \left(x_{t+1} + f_L\left(w^-_i\right)\right).
%$$
%
%



For  $i\in \{1,2,3,4,5,6\}$ define
$$
G_{(i)}(\alpha) =
\left\{
\begin{array}{ll}
\mbox{undefined} & \mbox{If $\alpha \not\in   \mathcal{I}^{(i)}$ }\\
\frac 1 2 \left( f_R(\alpha I^{(i)}_2(\alpha)  +  f_L(\alpha^{(i)}_1(\alpha))\right) &\mbox{If $\alpha \in   \mathcal{I}^{(i)}$ }  \\
\end{array}
\right.
$$
These  $G_{(i)}(\alpha)$  are therefore also piecewise linear functions that can be built in $O(n)$ time and have $O(n)$ inflection points.
%{\color{red}  This is not hard to prove but tedious}

Finally, define

$$
G_{(7)}(\alpha) =
\left\{
\begin{array}{ll}
\mbox{undefined} & \mbox{If no good pair Case 7 $\alpha_1,\alpha_2$ with $\alpha_1 + \alpha_2 = \alpha$ exists}\\
\frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1)) &\mbox{If good Case 7 pair $\alpha_1,\alpha_2$ with $\alpha_1 + \alpha_2 = \alpha$ exists}
\end{array}
\right.
$$
The ``undefined'' values in the first line will be allowed to be either explicitly undefined or assigned a value  $\frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1))$ for some arbitrary $\alpha_1,\alpha_2$ such that $\alpha_1+\alpha_2 = \alpha.$ Note that in this second case there will be some $i<7$ such that  $G_{(i)}(\alpha) < G_{(7)}(\alpha).$

We will now show that $G_{(7)}(\alpha) $  is a piecewise linear function can be built in $O(n)$ time and has $O(n)$ inflection points.
Since
$$G(\alpha) = \min_{1 \le i \le 7} G_{(i)}(\alpha)$$
(where the minimum is only taken over the functions defined at $\alpha$) this would imply  that $G(\alpha)$ is a piecewise linear function that can be built in $O(n)$ time and has $O(n)$ inflection points and thus $B'_t$ can be evaluated in $O(n)$ time via \Cref{eq:FG2replace}.


It thus remains to construct  $G_{(7)}(\alpha).$   Our approach will be to show that if  $(\alpha_1,\alpha_2)$ is a good Case 7 pair then either
$\alpha_1$ is an inflection point of $f_L(\alpha)$ or $\alpha_2$ is an inflection point of $f_R(\alpha)$.  This will permit restricting the   $(\alpha_1,\alpha_2)$  pairs that need to be examined.




We first  claim that it is impossible for a good Case 7 $(\alpha_1,\alpha_2)$   pair  to  simultaneously satisfy the following  3 conditions:
\begin{enumerate}
%\item[A1]  $\alpha_1 < w^+_i$ and $\alpha_2 > w^-_j$
\item[A1] $\exists \epsilon_L >0$ such that  $\epsilon_L < w^+_i - \alpha_1$ and $\forall \alpha \in [\alpha_1, \alpha_1 + \epsilon_L],$  $f_L(\alpha) = m_L \alpha + \beta_L.$
\item[A2] $\exists \epsilon_R >0$ such that $\epsilon_R < \alpha_2 - w^-_j$ and   $\forall \alpha \in [\alpha_2 -\epsilon_R, \alpha_2],$  $f_R(\alpha) = m_R \alpha + \beta_R.$
\item[A3] $m_L < m_R.$
\end{enumerate}
%(A1) is just stating that the worst case is not already covered by Cases (2) and (3).
Recall that $f_L$ and $f_R$ are piecewise linear functions with increasing slopes and $O(n)$ inflection points. In  (A1),  $m_L$  is the slope of $f_L$ at $\alpha_1$ as approached from the right; in  (A2),  $m_R$ is the slope of $f_R$ at $\alpha_2$ as approached from the left.


\medskip

Suppose that $A1$-$A3$ are simultaneously valid  for some  good $(\alpha_1, \alpha_2)$ case 7 
pair and set $y = y(\alpha_1,\alpha_2).$   % and also that  $y=y(\alpha_1,\alpha_2)\not=x_t$.
Because it is a case 7 pair with $y \in \bar I_t$,  $y > x_t.$
Set $\delta > 0$ such that $\delta < \min \left\{ \epsilon_L,\, \epsilon_R, \frac {2 (y-x_t)} {m_R +m_L} \right\}$
%For small enough $\delta > 0$
and then set $\alpha'_1 = \alpha_1 + \delta$ and $\alpha'_2 = \alpha_2 - \delta.$
Then 
$$f_L(\alpha'_1) = f_L(\alpha_1) + \delta m_L,\quad
f_L(\alpha'_2) = f_L(\alpha_2) - \delta m_R.
$$
Thus, from \Cref{eq:yalph}, 
$$y(\alpha'_1, \alpha'_2) = \frac 1 2 ( f_R(\alpha'_2)  -  f_L(\alpha'_1)) = y - \frac \delta 2 (m_L + m_R) > x_t
$$
so $y(\alpha'_1,\alpha'_2) \in I_t.$ 
On the other hand, $\alpha'_1+ \alpha'_2= \alpha_1+ \alpha_2$ and 
$$\frac 1 2 ( f_R(\alpha'_2)  +  f_L(\alpha'_1)) 
= \frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1)) + \frac 1 2 (m_L - m_R) < \frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1))
$$
 contradicting  the fact that $\alpha_1, \alpha_2$ is a good pair. Thus $A1$-$A3$ can not be  simultaneously valid  for some  good $(\alpha_1, \alpha_2)$ case 7 
pair.
 


By a symmetric argument we also see that  it is impossible for a good Case 7 $(\alpha_1,\alpha_2)$   pair  to  simultaneously satisfy the following  3 conditions:
\begin{enumerate}
%\item[B1]   $\alpha_2 < w^+_j$ and $\alpha_1 > w^-_i$
\item[B1]  $\exists \epsilon_R >0$ such that  $\epsilon_R < w^+_j - \alpha_2$ and $\forall \alpha \in [\alpha_2, \alpha_2 + \epsilon_R],$  $f_R(\alpha) = m_R \alpha + \beta_R.$
\item[B2]  $\exists \epsilon_L >0$ such that $\epsilon_L < \alpha_1 - w^-_1$ and   $\forall \alpha \in [\alpha_1 -\epsilon_L, \alpha_1],$  $f_L(\alpha) = m_L \alpha + \beta_L.$
\item[B3]  $m_R < m_L.$
\end{enumerate}


Suppose now that neither $\alpha_1$ nor $\alpha_2$ are inflection points, respectively, of $f_L$ and $f_R$,
$\alpha_1 \not=w_i^-,w_i^+$ and   $\alpha_2 \not=w_j^-,w_j^+$.
Then A1, A2, B1, B2 are all valid.
 
 Furthermore, if  $m_L \not = m_R$ then exactly  one of A3, B3 is true, leading to a contradiction.

Now suppose   $m_L  = m_R$  and  define   $\alpha'_1 = \alpha_1 + \delta$ and $\alpha'_2 = \alpha_2 - \delta$ for some $\delta>0$  to be set soon. The same calculations as above show that, as long as $\alpha'_1$ remains on the same line segment for $f_L(\alpha)$ as $\alpha_1$ and  $\alpha'_2$ stays on the same line segment for $f_L(\alpha)$ as $\alpha_2$
$$y(\alpha'_1, \alpha'_2) = \frac 1 2 ( f_R(\alpha'_2)  -  f_L(\alpha'_1)) = y - \frac \delta 2 (m_L + m_R)  = y - \delta m_L
$$
and
$$\frac 1 2 ( f_R(\alpha'_2)  +  f_L(\alpha'_1)) 
= \frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1)) + \frac 1 2 (m_L - m_R) = \frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1)).
$$
Note that  $\alpha'_1 + \alpha'_2 = \alpha_1 + \alpha_2$.

Now start with $\delta=0$ and smoothly increase $\delta$ until the first time one of the following occurs: (i) $\alpha'_1 = w_i^+,$  (ii) $\alpha'_2 = w_j^-$,  (iii) $y(\alpha'_1,\alpha_2) = x_t$,  (iv) $\alpha'_1$ is an inflection point of $f_L(\alpha)$ or (v)   $\alpha'_2$ is an inflection point of $f_R(\alpha).$   By construction one of these must occur.  The resulting
$(\alpha'_1, \alpha'_2)$ also has  $y(\alpha'_1, \alpha'_2) \in I_t$ and has the same cost as $(\alpha_1, \alpha_2)$ and is therefore also a good pair for $\alpha= \alpha_1 + \alpha_2.$

If (i) occurs, then  $(\alpha'_1, \alpha'_2)$  is a good Case 2 pair and would have apeared as $G_2(\alpha).$   If (ii) occurs it is a good Case (3) pair and would have appeared as $G_3(\alpha).$     If (iv) occurs, it is a good Case (5) pair and would have appeared as $G_5(\alpha).$   



We have therefore just seen that if $G_7(\alpha)$ is defined but $G_2(\alpha)$, $G_3(\alpha)$ and $G_5(\alpha)$ is not defined  then 
$G_{(7)} (\alpha) = \frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1))$   where at least one of $\alpha_1$ or $\alpha_2$ is an inflection point.



We now describe how this permits $O(n)$ construction of $G_{(7)}(\alpha)$, a piecewise linear function with $O(n)$ inflection points.  This in turn permits the 
$O(n)$ construction of $G(\alpha)$, a piecewise linear function with $O(n)$ inflection points which in turn permits the evaluation of 
\Cref{eq:FG2replace} in $O(n)$ time.



\medskip
From the discussion above we may assume that, in Case 7,  at least one of $\alpha_1$ and $\alpha_2$ are inflection points,  $\alpha_1 \not=w_i^-,w_i^+$ and   $\alpha_2 \not=w_j^-,w_j^+$ (since those are dealt with by the other cases).

\medskip

Now let $m_{L_1} < m_{L_2} < \cdots   < M_{L_t}$ be the slopes defining the line segments of $F_L(\alpha)$ for $\alpha \in [w_i^-,w^i+].$
Similarly let 
 $m_{R_1} < m_{R_2} < \cdots   < M_{R_u}$ be the slopes defining the line segments of $F_R(\alpha)$ for $\alpha \in [w_j^-,w^j+].$
 The inflection  points of  $F_L(\alpha)$ in $ [w_i^-,w^i+]$ are exactly the $t-1$ points,  $k=1,\ldots, u-1$,  $\alpha^L_k$ where $\alpha^L_k$ is the intersection of the line with slope
 $m_{L_k}$ and $m_{L_{k+1}}.$
 
 Similarly, the inflection  points of  $F_R(\alpha)$ in $ [w_j^-,w_j^+]$ are exactly the $u-1$ points,  $r=1,\ldots, t-1$,  $\alpha^R_r$ where $\alpha^R_r$ is the intersection of the line with slope
 $m_{R_r}$ and $m_{R_{r+1}}.$
 
 \medskip
 
\par\noindent{\bf First suppose that ($\alpha^L_k,\alpha^R_r)$  is a good Case 7 pair where both $\alpha^L_k$  and   $\alpha^R_r$ are inflection points. }

\medskip
We are given that it is impossible for all of A1-A3 to be simultaneously  valid and that  it is also impossible for all of B1-B3 to be simultaneously  valid 


%  Let $m_{L_1} < m_{L_2}$ be the two slopes of the lines intersecting to form $f_L$ at $\alpha_1$  and $m_{R_1} < m_{R_2}$ be the two slopes of the lines intersecting to form $f_R$ at $\alpha_2.$  
  
  \medskip
  
  
  Conditions A1-A3 not being valid implies $m_{R_r}\le m_{L_{k+1}}$ and   conditions B1-B3 not being valid implies $m_{L_k}\le m_{R_{r+1}}$.  If $m_{L_{k}} = \min\{m_{L_k},m_{R_r}\}$ this implies either  
\begin{equation}
\label{eq:aa1}
m_{L_k} \le m_{R_r} < m_{R_{r+1}} \le m_{L_{k+1}}
\end{equation}
or
\begin{equation}
\label{eq:aa2}
m_{L_k} \le m_{R_r} \le m_{L_{k+1}} \le m_{R_{r+1}}
\end{equation}
where, in the last equation, at least one of the first two $\le$ is a $<$ and at least one of the last two $\le$ is a $<.$
Similarly, if  $m_{R_{r}} = \min\{m_{L_{k}},m_{R_{r}}\}$ this implies either  
\begin{equation}
\label{eq:aa3}
m_{R_{r}} \le m_{L_{k}} < m_{L_{k+1}} \le m_{R_{r+1}}
\end{equation}
or
\begin{equation}
\label{eq:aa4}
m_{R_{r}} \le m_{L_{k}} \le m_{R_{r+1}} \le m_{L_{k+1}}
\end{equation}
where, in the last equation, at least one of the first two $\le$ is a $<$ and at least one of the last two $\le$ is a $<.$
If one of \Cref{eq:aa1,eq:aa2,eq:aa4,eq:aa4} occurs, we say that $\alpha^L_k$ and $\alpha^R_r$ can be {\em matched}.


From the conditions,  if  $\alpha^{R_r}$ and if  $\alpha^{R}_{r''}$ with $r < r''$ are both matched with  $\alpha^L_k$ then  $\alpha^{R}_{r'}$ is also matched with $\alpha^L_k$ for all $r < r' < r''.$

Similarly, if  $\alpha^{L_k}$ and if  $\alpha^{L}_{k''}$ with $k < k''$ are both matched with  $\alpha^R_r$ then  $\alpha^{L}_{k'}$ is also matched with $\alpha^R_r$ for all $k < k' < k''.$


%
%there are $O(n)$ possible such pairs
%
%{\color{red} This needs more}

%
% This implies that if inflection points are sorted by the slope of their incoming edge from below,  only $(\alpha_1,\alpha_2)$ pairs that are consecutive inflection points in the sorted order can be a good pair that defines $G_{(7)}(\alpha).$


\medskip

\par\noindent{\bf Now suppose that ($\alpha^L_k,\alpha_2)$  is a good Case 7 pair,  where  $\alpha_2$ is not an inflection point.}

Let  $m_{R_r}$ be the slope of the line in $f_R$ on which $\alpha_2$ lies.

If $m_{L_{k+1}} < m_{R_r}$ then  all of A1-A3 are satisfied, leading to a contradiction.  

If $m_{R_r} < m_{L_{k}}$ then  all of B1-B3 are satisfied, leading to another contradiction.

Thus,  $m_{L_{k}}  \le m_{R_r} \le m_{L_{k+1}}$.
Note that for any given  edge in $f_{R}$ this implies that there is a unique inflection point $\alpha^L_k$ in $f_L$ with which $\alpha_2$ on that edge can be ``matched''.

\medskip

Recall that the inflection points $\alpha^R_{r-1}$, $\alpha^R_{r}$ are the endpoints of the edge with slope $m_{R_r}$(unless the edge is the first or last edge in the range of $f_R,$ in which case only the second or first is an endpoint and the other endpoint is $w^-_j$ or $w^+_j$).  $m_{L_{k}}  \le m_{R_r} \le m_{L_{k+1}}$ implies that the pair $(\alpha^L_k,\alpha^R_{r-1})$ satisfies one of the two conditions  \Cref{eq:aa1,eq:aa4}  and  the pair $(\alpha^L_k,\alpha^R_{r})$ satisfies one of the two conditions  \Cref{eq:aa2,eq:aa3}. 
Thus, the two endpoints of the edge can also be matched with $\alpha^L_k$.  By a similar argument, if the edge is the first or last edge, its unique inflection point endpoint can be matched with $\alpha^L_k.$


Note that in the other direction, if both $\alpha^R_{r-1}$, $\alpha^R_{r}$ can be matched with $\alpha^L_{k}$ then the edge of $f_R$'s for which they are the endpoints  has slope $m_{R_r}$ and thus can be matched with $\alpha^L_{k}$.  The first edge in  $f_R$  has endpoints $w^-_j$ and $\alpha^R_1$.  It can only be matched with the unique inflection  point (if it exists) $\alpha^L_k$ such that $m_{L_{k}}  \le m_{R_1} \le m_{L_{k+1}}$.
Similarly the last edge  in  $f_R$  has endpoints $\alpha^R_{u-1}$ and $w^+_j$ 
  It can only be matched with the unique articulation point (if it exists) $\alpha^L_k$ such that $m_{L_{k}}  \le m_{R_{u-1}} \le m_{L_{k+1}}$.


\medskip

Given any inflection point $\alpha^L_k$, let $\alpha^R_r,\, \alpha^R_{r+1},\ldots,\alpha^R_{r''}$ be the contiguous set of inflection points that are matched with  
$\alpha^L_k$.  This corresponds to the $r''-r$ edges of $f_R$ that have those inflection points as endpoints.  
\begin{enumerate}
\item Set $A_2(\alpha^L_k) = [\alpha^R_r,\alpha^R_{r''}]$; this is   the union of those edges.  
\item If $\alpha^L_k$ matches to $\alpha^R_1$ append $[w^-_j,\alpha^R_1]$ to the front of $A_2(\alpha^L_k)$
\item  If $\alpha^L_k$ matches to $\alpha^R_{u-1}$ append $[\alpha^R_{u-1},w^+_j]$ to the end of $A_2(\alpha^L_k)$. 
\end{enumerate}
Note two special cases for step 1:  if $r=r'$ then  $A_2(\alpha^L_k)$ is exactly one point and if no $\alpha^R_r$ matches with $\alpha^L_k$ then $A_2(\alpha^L_k)$  is the empty set.


From the arguments above $A_2(\alpha^L_k)$ is exactly the set of $\alpha_2$ that can match with $\alpha^L_k.$
Also from the arguments above,  
two such sets can therefore not intersect except, possibly at one overlapping endpoint (which would be an inflection point of $f_R$). 
Also note that the creation of  $A_2(\alpha^L_k)$ can be done in $O(n)$ time using a linear scan through the two function representations.



 
Now suppose that $\alpha^L_{k_1}$ and $\alpha^L_{k_2}$ are two inflection points with $k_1 < k_2$. Since the supporting line slopes of  $A_2(\alpha^L_{k_1})$ are less than the supporting line slopes  $A_2(\alpha^L_{k_2})$  these two sets can not intersect except, possibly at a unique overlapping inflection point of $f_R$.

This immediately implies that 
$$ \mbox{if $k_1 < k_2$,\ $\alpha_2 \in A_2(\alpha^L_{k_1})$ and $\alpha_2' \in A_2(\alpha^L_{k_2})$} 
\quad \Rightarrow \quad
\alpha^L_{k_1} + \alpha_2  < \alpha^L_{k_2} + \alpha_2'.
$$
This immediately implies that any value $\alpha$ can only have at most one good pair $\alpha_1 + \alpha_2 = \alpha$ where $\alpha_1$ is an inflection point.


Finally, given $\alpha^L_k$ and $\alpha_2 \in A_2(\alpha^L_k)$, another condition that must be satisfied is that
$$x_t \le  \bar y(\alpha^L_k,\alpha_2) \le  x_{t+1}$$
where $ \bar y(\alpha^L_k,\alpha_2) =  \frac 1 2 ( f_R(\alpha_2)  -  f_L(\alpha^L_k)).$ This can be rewritten as
$$ 2 x_t + f_L(\alpha^L_k) \le  f_R(\alpha_2) \le  2 x_{t+1} + f_L(\alpha^L_k).$$
Now define 
$$\bar A_2(\alpha^L_k) = \Bigl\{ \alpha_2  \in A_2(\alpha^L_k) \,:\,  2 x_t + f_L(\alpha^L_k) \le f_R(\alpha_2) \le  2 x_{t+1} + f_L(\alpha^L_k) \Bigr\}.
 $$
Note that $\bar A_2(\alpha^L_k)$ are also intervals and they can be created from the $ A_2(\alpha^L_k)$ in total $O(n)$ time.





Combining the above we see that if  $G_{(7)}(\alpha)$ exists  and is defined by a pair $\alpha = \alpha_1 + \alpha_2$ where $\alpha_1$  is an  inflection point  then it is the unique pair with $\alpha_2 = \alpha- \alpha_1 \in \bar A_2(\alpha_1).$ 
\medskip

We therefore may define the following ``function''

$$
G_{(7)}^L(\alpha) =
\left\{
\begin{array}{ll}
\frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha^L_k) &\mbox{If  $\alpha= \alpha^L_{k} + \alpha_2$  for some $k$ and $\alpha_2 \in \bar A_2(\alpha^L_k)$}\\
\mbox{undefined} & \mbox{If no such decomposition exists}\\
\end{array}
\right.
$$
From the arguments above every $\alpha$ has at most one such decomposition so this is well defined.  This function can be constructed in $O(n)$ time.  The construction will partition the $\alpha_2$ line into $O(n)$ intervals.  In each interval,  $G_{(7)}^L(\alpha)$ will either be defined by one linear function or will be undefined.


\medskip

\par\noindent{\bf Now suppose that ($\alpha_1, \alpha^R_r)$  is a good Case 7 pair,  where  $\alpha_1$ is not an inflection point.}
Now apply the same argument as above , flipping the roles of $f_L$ and $f_R.$


Given any inflection point $\alpha^R_r$, let $\alpha^L_k,\, \alpha^L_{k+1},\ldots,\alpha^L_{k''}$ be the contiguous set of inflection points that are matched with  
$\alpha^R_r$.  This corresponds to the $k''-k$ edges of $F_L$ that have those inflection points as endpoints.  
\begin{enumerate}
\item Set $A_1(\alpha^R_r) = [\alpha^L_k,\alpha^L_{k''}]$; this is   the union of those edges.  
\item If $\alpha^R_r$ matches to $\alpha^L_1$ append $[w^-_i,\alpha^L_1]$ to the front of $A_1(\alpha^R_r)$
\item  If $\alpha^R_r$ matches to $\alpha^L_{t-1}$ append $[\alpha^L_{t-1},w^+_i]$ to the end of $A_1(\alpha^R_r)$. 
\end{enumerate}
Following the derivation for the previous case $A_1(\alpha^R_r)$ is exactly the set of $\alpha_1$ that can match with $\alpha^R_r.$

We then define
$$\bar A_1(\alpha^R_r) = \Bigl\{ \alpha_1  \in A_1(\alpha^R_r) \,:\,  2 x_t + f_R(\alpha^R_r) < f_L(\alpha_1) < 2 x_{t+1} + f_L(\alpha^R_r) \Bigr\}
 $$
where  $\bar A_1(\alpha^R_r)$ is also an interval.



$$
G_{(7)}^R(\alpha) =
\left\{
\begin{array}{ll}
\frac 1 2 ( f_R(\alpha^R_r)  +  f_L(\alpha_1) &\mbox{If  $\alpha=   \alpha_1 + \alpha^R_{r}$  for some $r$ and $\alpha_1 \in A_1(\alpha^R_r)$}\\
\mbox{undefined} & \mbox{If no such decomposition exists}\\
\end{array}
\right.
$$
From the arguments above every $\alpha$ has at most one such decomposition so this is well defined.  This function can be constructed in $O(n)$ time.  The construction will partition the $\alpha_21$ line into $O(n)$ intervals.  In each interval,  $G_{(7)}^L(\alpha)$ will either be defined by one linear function or will be undefined.

\medskip

\par\noindent{\bf Concluding the proof.}

Recall that it only remained to show that 
 $G_{(7)}(\alpha) $  is a piecewise linear function that can be built in $O(n)$ time and has $O(n)$ inflection points. w e can do this by setting
  $G_{(7)}(\alpha)  = \bar  G_{(7)}(\alpha) $  where.
 $$\bar G_{(7)}(\alpha) = 
\left\{
\begin{array}{cl}
\mbox{undefined} & \mbox{ if both $G_{(7)}^L(\alpha)$ and  $G_{(7)}^R(\alpha)$ are undefined}\\
G_{(7)}^L(\alpha) &\mbox{ if  $G_{(7)}^L(\alpha)$  is defined  and  $G_{(7)}^R(\alpha)$ is undefined}\\
G_{(7)}^R(\alpha) &\mbox{ if  $G_{(7)}^L(\alpha)$  is undefined  and  $G_{(7)}^R(\alpha)$ is defined}\\
\min\left( G_{(7)}^L(\alpha),\, G_{(7)}^R(\alpha)\right) & \mbox{ if both $G_{(7)}^L(\alpha)$ and  $G_{(7)}^R(\alpha)$ are undefined}\\
\end{array}
\right.
$$

From the arguments above we know that if   $(\alpha_1,\alpha_2)$  is a good Case 7 pair for $\alpha$ then  there exists a good case 7 pair $(\alpha'_1,\alpha'_2)$ for $\alpha$  where at least one of $\alpha_1',\alpha_2'$ are inflection points.

To see that 
$G_{(7)}(\alpha)  = \bar  G_{(7)}(\alpha) $ note that  if no good Case 7 pair for $\alpha$ exists then $\bar  G_{(7)}(\alpha)$ is either undefined or equals
$\frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1))$ for some  $\alpha_1+\alpha_2 = \alpha$  and thus satisfies the conditions on $G_{(7)}(\alpha)$.

if a  good Case 7 pair for $\alpha$ exists then from  the arguments above we know that there exists a good case 7 pair $(\alpha'_1,\alpha'_2)$ for $\alpha$  where at least one of $\alpha_1',\alpha_2'$ are inflection points. Thus at least one of $G_{(7)}^L(\alpha)= G_{(7)}(\alpha)$ and $G_{(7)}^R(\alpha)= G_{(7)}(\alpha)$ must be true.

If  $G_{(7)}^L(\alpha) = G_{(7)}(\alpha)$   and  $G_{(7)}^R(\alpha) \not=  G_{(7)}(\alpha)$  then either $G_{(7)}^R(\alpha)$ is undefined and  trivially $G_{(7)}(\alpha)  = \bar  G_{(7)}(\alpha) $ or   $G_{(7)}^R(\alpha)$ is defined and  $G_{(7)}^R(\alpha)= \frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1))$ for some  $\alpha_1+\alpha_2 = \alpha$.  This would imply that 
$$ G_{(7)}^L(\alpha) = G_{(7)}(\alpha) < G_{(7)}^R(\alpha)$$
so 
$$\bar  G_{(7)}(\alpha)  = G_{(7)}^L(\alpha) = G_{(7)}(\alpha) .$$
A symmetric argument shows that
if  $G_{(7)}^R(\alpha) = G_{(7)}(\alpha)$   and  $G_{(7)}LR(\alpha) \not=  G_{(7)}(\alpha)$ then 
$$\bar  G_{(7)}(\alpha)  = G_{(7)}^R(\alpha) = G_{(7)}(\alpha) .$$
The final case is when $G_{(7)}^R(\alpha) = G_{(7)}(\alpha) =G_{(7)}LR(\alpha).$  In this case
trivially  $\bar  G_{(7)}(\alpha)  = G_{(7)}(\alpha)$ so we are done.




{\color{blue}

*****************
Not NEEDED and should be removed in final version

The case of  both being defined but not being equal to each other can no happen.  The proof (below) is long though and we don't need it.


$$G_{(7)}(\alpha)=
\min\left\{
\frac 1 2 ( f_R(\alpha_2)  +  f_L(\alpha_1)),\,
\frac 1 2 ( f_R(\alpha'_2)  +  f_L(\alpha'_1))\right\}.
$$
We show in this case that
$$ f_R(\alpha_2)  +  f_L(\alpha_1)= 
 f_R(\alpha'_2)  +  f_L(\alpha'_1)$$
so the two possible candidate solutions are both good and yield the same answer.






\medskip

If $\alpha'_1$ is an inflection point then, from the previous arguments, the two solutions would be unique.  Similarly, if $\alpha_2$ is an inflection point,  the two solutions would be the same.  We therefore assume that neither $\alpha'_1$  or  $\alpha_2$  is an inflection point.

Let $\alpha_1$ be defined by slopes $m_{L_1} < m_{L_2}$,  $\alpha'_2$ be defined by slopes $m_{R_1} < m_{R_2},$
$\alpha'_1$ on a line with slope $m_L$ and $\alpha_2$ on a line with slope $m_R$. Since  $\alpha'_1$  and  $\alpha_2$ are not inflection points, $m_L$  and $m_R$ are uniquely defined.

We know that $m_{L_1} \le m_R \le  m_{L_2}$ and $m_{R_1} \le m_L \le  m_{R_2}$.

Now, if $\alpha'_1 > \alpha_1$ then $\alpha'_2 < \alpha_2$.  This implies   $m_{L_2} \le m_L$   and $m_{R_2} \le m_R$.

The inequalities then combine to prove that
$$m_{L_1} \le m_R \le  m_{L_2} \le m_L
\quad\mbox{and}\quad m_{R_1} \le m_L \le  m_{R_2}\le m_R
$$
so
$$ m_R= m_L = m_{L_2} = m_{R_2}$$
(which also implies $m_{L_1} < m_{R}$ and $m_{R_1} < m_{L}).$ Set $m= m_L.$

Note that this means that $\alpha'_1$ is on the line segment that has  inflection point $\alpha_1$ as its left endpoint.
Similarly $\alpha_2$ is on the line segment that has  inflection point $\alpha'_2$ as its left endpoint.
Thus 
\begin{eqnarray*}
f_L(\alpha'_1) - f_L(\alpha_1)  &=& m(\alpha'_1 - \alpha_1)\\
&=& m(\alpha'_2 - \alpha_2)\\
&=& f_R(\alpha'_2) - f_R(\alpha_2) 
\end{eqnarray*}
proving
$$ f_R(\alpha_2)  +  f_L(\alpha_1)= 
 f_R(\alpha'_2)  +  f_L(\alpha'_1).$$


\medskip

The arguments above show that  if there are two possible candidate solutions they both provide the same answer.

Therefore,  for every inflection point $\alpha_1$ and every $\alpha_2 \in \bar A_2(\alpha_1),$ and also for  for every inflection point $\alpha_2$ and every $\alpha_1 \in \bar A_1(\alpha_2),$
$$G_{(7)}(\alpha_1 + \alpha_2) = \frac 1 2 f_L(\alpha_1)+  \frac 1 2 f_R(\alpha_2).$$

**************************
}

\end{proof}


\subsection{Efficient Computation of $R_{\max}(P,x)$}





Combining \Cref{thm:reduction3} with  \Cref{lem:bar construction,cor:GH}
 immediately gives a method for calculating  $R_{\max}(P,x)$
 in $O(n^4 )$ time for any fixed $x.$


\subsection{Calculating $R_{OPT}(P)$}

Let $x^*$ be the sink location such that $R_{OPT}(P) =R_{\max}(P,x^*)$.
From \Cref{lem:rmax unimodal}, $R_{\max}(P,x^*)$ is a unimodal function so, from \Cref{obs:bs unimodal},  using $O(\log n)$ queries, we can find 
 index $u$ such that $x_u \le x^* \le  x_{u+1}$.  Recall that a query is the evaluation of $R_{\max}(P,x)$ for a fixed $x,$ which we just saw can be done in $O(n^4)$ time.
So, finding $u$ can be done in  $O(n^4 \log n)$ time.

After this process we know $u,$  $R_{\max}(P,x_u)$ and $R_{\max}(P,x_{u+1})$.

Next note that, for  $x_u < x <  x_{u+1}$, if we define  $\delta = x - x_u,$ then, for  $x_j \le x$ and  
$x \le x_i$,
and  the definition of $g_j(x,s)$ in \Cref{cor:smooth evac}
$$
g_j(x:s) = g_j(x_{u+1}:s) - (d_u - \delta),
\quad\mbox {and}\quad
h_i(x:s) = g_j(x_{u}:s) - \delta.
$$
Plugging into \Cref{def:gandh defs} yields 
\begin{align}
G_{j} (x) &=\max_{ s \in S_{j,j}} \left\{ g_j(x:s) - \min_{y \ge x_j} \Theta(P,y:s)  \right\}
=  G_{j} (x_{u+1})- (d_u - \delta),\\
H_{i} (x) &=   \max_{ s \in S_{i,i}} \left\{ h_i(x:s) - \min_{y \le x_i} \Theta(P,y:s) \right\}
= H_{i}(x_u) - \delta
\end{align}
Similarly, we find
\begin{eqnarray*}
G_{i,j}(x) &=&  G_{i,j}(x_{u+1}) -(d_u - \delta),\\
\bar G_{i,j}(x) &=&  G_{i,j}(x_{u+1}) -(d_u - \delta),\\
H_{i,j}(x)  &=& H_{i,j}(x_u) - \delta\\
\bar H_{i,j}(x)  &=& H_{i,j}(x_u) - \delta.
\end{eqnarray*}
Plugging this into \Cref{thm:reduction3} yields
$$R_{\max}(P,x) =\max  \left\{   A(u) - (d_u - \delta),\,  B(u) -\delta  \right\} 
$$
where 
\begin{eqnarray*}
A(u) &=&\max \left\{
\max_{\substack{j \\{x_j \le x_u}}}   G_{j}(x_{u+1}),
\max_{\substack{i < j \\{ x_j \le x_u}}}   G_{i,j}(x_{u+1}),
\max_{\substack{i < j \\{x_j \le x_u}}} \bar G_{i,j}(x_{u+1}),
\right\} \\
B(u) &=&\max \left\{
\max_{\substack{ i\\ {x_{u+1} \le x_i }}} H_{i}(x_u),
\max_{\substack{i < j \\ {x_{u+1} \le x_i }}} H_{i,j}(x_u),
\max_{\substack{i < j \\ {x_{u+1} \le x_i }}}  \bar H_{i,j}(x_u)
\right\} 
\end{eqnarray*}
Using the previous lemmas,  $A(u)$ and $B(u)$ can be calculated in $O(n^4 \log n)$  
  
  Also notice that, by definition $A(u) - d_u \le R_{\max}(P,x_u)$ and
  $B(u) \le R_{\max}(P,x_{u+1})$.
  Thus
  
  $$ R_{OPT}(P) =
  \max \left\{
  R_{\max}(P,x_u),\, 
  \max_{0 \le \delta \le d_u} \max  \left\{   A(u) - (d_u - \delta),\,  B(u) -\delta  \right\}'\, 
   R_{\max}(P,x_{u+1})
  \right\}
  $$
  which can be calculated in an additional $O(1)$ time and we are finished.
  



